A General Path-Based Representation for Predicting Program Properties

Predicting program properties such as names or expression types has a wide range of applications. It can ease the task of programming and increase programmer productivity. A major challenge when learning from programs is $\textit{how to represent programs in a way that facilitates effective learning}$. We present a $\textit{general path-based representation}$ for learning from programs. Our representation is purely syntactic and extracted automatically. The main idea is to represent a program using paths in its abstract syntax tree (AST). This allows a learning model to leverage the structured nature of code rather than treating it as a flat sequence of tokens. We show that this representation is general and can: (i) cover different prediction tasks, (ii) drive different learning algorithms (for both generative and discriminative models), and (iii) work across different programming languages. We evaluate our approach on the tasks of predicting variable names, method names, and full types. We use our representation to drive both CRF-based and word2vec-based learning, for programs of four languages: JavaScript, Java, Python and C\#. Our evaluation shows that our approach obtains better results than task-specific handcrafted representations across different tasks and programming languages.

==> featuregen - Copy/abstract3.tex <==
\begin{abstract}
Predicting program properties such as names or expression types has a wide range of applications. It can ease the task of programming, and increase programmer productivity. A major challenge when learning from programs is \emph{how to represent programs in a way that facilitates effective learning}.

We present a \emph{general path-based representation} for learning from programs. Our representation is purely syntactic and extracted automatically. The main idea is to represent a program using paths in its abstract syntax tree (AST). This allows a learning model to leverage the structured nature of code rather than treating it as a flat sequence of tokens.

We show that this representation is general and can:
\begin{inparaenum}[(i)]
\item cover different prediction tasks,
\item drive different learning algorithms (for both generative and discriminative models), and
\item work across different programming languages.
\end{inparaenum}

We evaluate our approach on the tasks of predicting variable names, method names, and full types. We use our representation to drive both CRF-based and word2vec-based learning, for programs of four languages: JavaScript, Java, Python and C\#. Our evaluation shows that our approach obtains better results than task-specific handcrafted representations across different tasks and programming languages.
\end{abstract} 	

==> featuregen - Copy/acknowledgement.tex <==
\begin{acks}

We would like to thank Eytan Singher for implementing the C\# module of \tool.
We also thank Miltiadis Allamanis, Veselin Raychev and Pavol Bielik for their guidance in the use of their tools in the evaluation section.

The research leading to these results has received funding from the European Union's Seventh Framework Programme (FP7) under grant agreement no. 615688-ERC- COG-PRIME. Cloud computing resources were provided by a Microsoft Azure for Research award and an AWS Cloud Credits for Research award.

\hfill \break
\hfill \break

\end{acks} 

==> featuregen - Copy/application.tex <==
\section{AST Paths Representation}\seclabel{application}
In this section, we formally describe the family of AST paths.

\subsection{AST Paths}\seclabel{PathFeatures}
To learn from programs, we are looking for a representation that captures interesting properties of ASTs while keeping it open for generalization. One way to obtain such a representation is to decompose the AST to parts that repeat across programs but can also discriminate between different programs. One such decomposition is into paths between nodes in the AST. We note that in general we consider n-wise paths, i.e., those that have more than two ends, but for simplicity we base the following definitions on pairwise paths between AST terminals.


We start by defining an AST, an AST-path, a path-context and an abstract path-context.

\begin{definition}[Abstract Syntax Tree]
An Abstract Syntax Tree (AST) for a code snippet $\mathcal{C}$ is a tuple $\langle N, T, X, s, \delta, val \rangle$ where $N$ is a set of nonterminal nodes, $T$ is a set of terminal nodes, $X$ is a set of terminal values, $s\in N$ is the root node, $\delta: N\rightarrow \left(N\cup T\right)^*$ is a function that maps a nonterminal node to a list of its children, and $val:T\rightarrow X$ is a function that maps a terminal node to an associated value. Every node except the root appears exactly once in all the lists of children.
\end{definition}

For convenience, we also define $\pi:\left(N\cup T\right)\rightarrow N$, the inverse function for $\delta$. Given a node, this function returns its parent node, such that for every two terminal or nonterminal nodes $y_1,y_2\in\left(N\cup T\right)$, one is the parent node of the other if and only if the latter is in the list of children of the former: $\pi\left(y_1\right)=y_2\iff y_1\in \delta\left(y_{2}\right)$.
In the case of the start symbol, its parent is undefined.

Next, we define AST pairwise paths. For convenience, in the rest of this section we assume that all definitions refer to a single AST $ \langle N, T, X, s, \delta, val \rangle$.

An AST pairwise path is a path between two nodes in the AST, formally defined as follows:

\begin{definition}[AST path]
An AST-path of length $k$ is a sequence $n_{1}d_{1}...n_{k}d_{k}n_{k+1}$, where for $i\in \left[1..k+1\right]$: $n_{i}\in \left(N\cup T\right)$ are terminals or nonterminals and for $i\in \left[1..k\right]$:  $d_{i} \in \{ \uparrow, \downarrow\}$ are movement directions (either up or down in the tree). If $d_{i}=\uparrow$, then: $n_{i+1}=\pi\left(n_i\right)$; if $d_{i}=\downarrow$, then: $n_{i}=\pi\left(n_{i+1}\right)$. We use $start\left(p\right)$ to denote $n_{1}$ and $end\left(p\right)$ to denote $n_{k+1}$.
\end{definition}

We define a \emph{path-context} as a tuple of an AST path and the values associated with its end nodes: (i.e. $n_{1}$ and $n_{k+1}$). In general, we consider path-contexts which span between arbitrary AST nodes, e.g., a terminal and its ancestor, but for simplicity, we base the following definitions on path-contexts which span between terminals:

\begin{definition}[Path-context]
Given an AST Path $p$, its path-context is the triplet $\langle x_{s},p,x_{f} \rangle$ where $x_{s} = val\left(start\left(p\right)\right)$ and $x_{f} = val\left(end\left(p\right)\right)$ are the values associated with the start and end nodes of $p$.
\end{definition}

That is, a path-context describes two nodes from the AST with the syntactic path between them.

Finally, we define an \emph{Abstract path-context} as an abstraction of concrete path context:

\begin{definition}[Abstract path-context]
Given a path-context $\langle x_{s},p,x_{f} \rangle$ and an abstraction function $\alpha:P\rightarrow\hat{P}$,
an abstract path-context is the triplet $\langle x_{s},\alpha\left(p\right),x_{f} \rangle$,
where $P$ is the set of AST paths,
$\hat{P}$ is the set of abstract AST paths,
and $\alpha$ is a function that maps a path to an abstract representation of it.
\end{definition}

The abstraction function $\alpha$ is any function that transforms a path to a different representation. A trivial abstraction function is $\alpha_{id}$, which maps a path to itself: $\alpha_{id}\left(p\right)=p$.

\input{statementpath-figure}

\begin{example}
For example, consider the JavaScript line of code in~\figref{childIdExampleLine} and its partial AST in~\figref{statementPath}. We denote the path between the variable \scode{item} to the variable \scode{array} by $p$. Using $\alpha_{id}$, the abstract path-context of $p$ is:
\begin{align}
\small
&\langle \scode{item},\alpha_{id}\left(p\right),\scode{array} \rangle= \\
&\langle\scode{item},\left(SymbolVar\uparrow VarDef \downarrow Sub\downarrow SymbolRef\right),\scode{array}\rangle
\end{align}
Using a different abstraction function yields a different abstract path-context, for example $\alpha_{forget-arrows}$:
\begin{align}
\small
\langle & \scode{item},\alpha_{forget-arrows}\left(p\right),\scode{array} \rangle= \\
&\langle \scode{item}, \left(SymbolVar , VarDef , Sub , SymbolRef\right), \scode{array} \rangle
\end{align}
\end{example}

Na\"ively extracting all the paths in the AST and representing each of them uniquely can be computationally infeasible, and as a result of the bias-variance tradeoff~\cite[p.~37 and 219]{statisticalLearningBook}, can lead to worse prediction results. However, alternative abstraction functions can be used to control the number of distinct extracted paths. In~\secref{Abstractions} we describe alternative abstractions that abstract some of the information, and thus allow us to tune the trade-off between accuracy, training time, and model size.

\ignore{ % Ignoring the whole subject of child indices, it's an implementation detail which we don't want to include in the formal definition
\para{Path encoding}
When representing a path as a string, there are various ways to encode it. In this section, we describe a ``full'' path encoding that encodes all the information in the path.

In order to accurately capture the relationship a path represents, we encode it as a sequence of node types, separated by up and down symbols $\left\{\uparrow ,\downarrow\right\}$, indicating upward and downward movement between every two adjacent nodes.
Furthermore, different sibling nodes can have different semantic meanings, e.g. a function name and argument, an object and its field name, etc.
In order to differentiate between these roles, each node representation can include additional information.

Consider the JavaScript line of code in~\figref{childIdExampleLine} and its partial AST in~\figref{statementPath}. If the encoding of a path had been composed only of node types and up and down symbols, the path from the variable \scode{item} to the variable \scode{array} and from \scode{item} to \scode{i} would have been encoded as:
\begin{equation}
\textrm{SymbolVar }{\uparrow}\textrm{ VarDef }{\downarrow}\textrm{ Sub }{\downarrow}\textrm{ SymbolRef}
\equlabel{pathNoChildId}
\end{equation}
The roles of \scode{array} and \scode{i} are very different: \scode{array} is likely to represent an array while \scode{i} is likely to represent an index in the array, and we want our representation to capture this difference.
%; we want both \scode{array} and \scode{i} to uniquely affect the prediction of \scode{item}, and we want a model to be able to predict different names for \scode{array} and \scode{i} in accordance with the effect of \scode{item}
Therefore, for each node in the path, we add its \emph{child-index} --- the index of the node in the list of children of its parent node. Accordingly, the path from \scode{item} to \scode{array}, and the path from \scode{item} to \scode{i} are encoded as:
\begin{equation}
\footnotesize
\begin{split}
&\textrm{SymbolVar}_{\textbf{0}}\textrm{ }{\uparrow}\textrm{ VarDef}_{\textbf{0}}\textrm{ }{\downarrow}\textrm{ Sub}_{\textbf{1}}\textrm{ }{\downarrow}\textrm{ SymbolRef}_{\textbf{0}\textrm{ }}  \left(\scode{item}\rightarrow\scode{array}\right) \\
&\textrm{SymbolVar}_{\textbf{0}}\textrm{ }{\uparrow}\textrm{ VarDef}_{\textbf{0}}\textrm{ }{\downarrow}\textrm{ Sub}_{\textbf{1}}\textrm{ }{\downarrow}\textrm{ SymbolRef}_{\textbf{1}}\textrm{ } \left(\scode{item}\rightarrow\scode{i}\right)
\end{split}
\equlabel{pathWithChildId}
\end{equation}

Child-indices also differentiate between different arguments in a method invocation and different parameters in a method body.
}

\begin{figure}
\begin{subfigure}[b]{0.15\textwidth}
\centering
\lstset{language=JavaScript, basicstyle=\footnotesize\ttfamily,emph={fence},emphstyle=\underbar,showlines=true,escapeinside={(*@}{@*)}}
%\begin{tabular}{cc}
\begin{lstlisting}

var a, b, c, d;


\end{lstlisting}
%\end{tabular}
%\caption{An example of a JavaScript statement}
%\label{Fi:childIdExampleLine}
\end{subfigure}
\unskip \vrule
\hspace{1mm}
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includegraphics[width=2in]{length-width}
%\caption{The partial AST of the statement}
%\label{Fi:statementPath}
\end{subfigure}
\caption{An example statement and its AST, with an example of a path between the \emph{SymbolVar} terminals that represent \scode{a} and \scode{d}. The length of this path is $4$, and its width is $3$.}
\label{Fi:length-width}
\end{figure}

\subsection{Limiting the Number of Paths}\seclabel{ExtractingPaths}
Another approach for controlling the number of distinct paths is to limit the \emph{number of extracted paths}.

\para{Path length and width}
We define hyper-parameters that limit the path length and width. We define the following hyper-parameters:
\begin{itemize}
\item \maxlen, defined as the maximal \emph{length} of a path, i.e., the maximum value of $k$.
\item \maxwidth, defined as the maximal allowed difference between sibling nodes that participate in the same path, as shown in~\figref{length-width}.
\end{itemize}
When limiting these parameters to certain values, we do not extract longer or wider paths. We tune the optimal values of width and length by grid search of combinations on a validation set of programs and choose the combination that yields the highest accuracy, as described in~\secref{evaluation}. The tuning process of finding the optimal parameter values should be separate for each language and task.


Obviously, setting the values of these parameters to a value that is too low limits the expressiveness of the paths, does not capture enough context for each element, limits the ability to model the training and test data, and therefore produces poor accuracy. Why, then, does limiting the path length and width actually improve accuracy? There are several reasons:
\begin{itemize}
\item {\bfseries Locality} The role of a program element is affected mostly by its surroundings. For example, consider the program in~\figref{widthExample}. The width of a path that connects the variable \scode{a} in the first line to the variable \scode{b} in the last line is as large as the number of lines in the program. Usually, the names of \scode{a} and \scode{b} can be predicted by considering elements within a closer distance. Therefore, using paths between too distant elements can cause noise and pollute the relevant information.
\item {\bfseries Sparsity} Using paths that are too long can cause the representation space to be too sparse. A long path might appear too few times (or even only once) in the training set and cause the model to predict specific labels with high probability. This phenomenon is known as \emph{overfitting}, where the learned AST paths are very specific to the training data and the model fails to generalize to new, unseen data.
\item {\bfseries Performance} There is a practical limit on the amount of data that a model can be trained on. Too much data can cause the training phase to become infeasibly long. There is a tradeoff between how many programs the model can be trained on, and how many paths are extracted from each program. Therefore, it makes sense to limit the number of extracted paths from each program by limiting the paths' length and width, in order to be able to train on a larger and more \emph{varied} training set. %In practice, we found that for name prediction lengths of 6-7 and widths of 3-4 are both expressive enough and feasible. Other tasks require slightly different parameter values.
\end{itemize}

\begin{figure}
\centering
\lstset{language=JavaScript, basicstyle=\footnotesize\ttfamily,emph={fence},emphstyle=\underbar,escapeinside={(*@}{@*)}}
\begin{tabular}{cc}
\begin{lstlisting}
assert.equal(a,1);
assert.equal(...);
...
assert.equal(b,1);
\end{lstlisting}
\end{tabular}
%\caption{An example of a JavaScript statement}
%\label{Fi:childIdExampleLine}
\caption{An example of a typical program where the maximal path length is relatively small, but the width can be large.}
\label{Fi:widthExample}
\end{figure}

In fact, tuning path length and width is used to control the bias-variance tradeoff. Shorter paths increase the bias error, while longer paths increase the variance error. The relationship between these parameters and results is discussed and demonstrated in~\secref{hyperparams}.


==> featuregen - Copy/background.tex <==
\section{Background}\label{Se:background}
In this section, we provide necessary background.
%In~\secref{nlp} we present the use of path features in NLP
In Sections~\ref{Sec:crfs} and~\ref{Sec:w2v} we present CRFs and word2vec and how they are used to predict program properties.

%\subsection{Path Features in Natural Language Processing}\seclabel{nlp}

%A parse tree path in natural language is defined as the path from one word $w_x$ to another word $w_y$ along the syntactic parse tree of a given sentence, represented as a continuous string of parse tree nonterminals (in the case of constituency parsers) or terminals and their syntactic dependencies (in the case of dependency parsers). Several variations of these paths have also been introduced, such as ``partial paths'', ``shallow paths'', and ``subpaths'' \cite{Johansson2005}. While parse tree paths explicitly encode the syntactic connection between $w_x$ and $w_y$, they also encode important \emph{semantic} information implicitly. Hence, path features have been extensively used as features for addressing semantic tasks in natural language processing (NLP).

%One of the more prominent uses of path features is in semantic role labeling (SRL) \cite{gildeajurafsky2002}, where the goal is to associate semantic arguments with a particular target predicate (typically a verb). For example, in the sentence ``IQ tests are a common method of identifying gifted children'', the predicate ``identifying'' takes ``IQ tests'' as the \textit{instrument} argument. Understanding semantic roles is a fundamental challenge in NLP, and can be closely tied to question answering \cite{he2015qasrl}. %; for instance, understanding that IQ tests are the instrument of identification can answer the question ``What tools are used to identify gifted children?''
%While semantic roles go beyond syntax, parse tree paths have been shown to be powerful features in SRL systems.

%Another example of inferring semantics from syntactic paths is hypernymy detection. In this task, we are interested in classifying when one word $w_x$ is an instance or a subtype of another word $w_y$. For example, Toyota is a type of car manufacturer. \citet{snow2004learning} and later others \cite{turney2006similarity,shwartz2016improving} showed that certain syntactic paths are very discriminative of this relation, and that using the set of all path features between $w_x$ and $w_y$ yields robust hypernymy detectors. Syntactic paths were also used to capture word similarity via word2vec \cite{levy2014dependency}, by representing each word as a function of its syntactic relations with other words.

%Since programming languages are formal languages, their structural information is explicit, rich, and inherent. Even though natural language also has a structure, it tends to be less strict and more ambiguous. Therefore, a reasonable assumption is that using syntactic path features in programming languages can be even more advantageous than in natural language.

%One of the first uses of parse tree paths as features was in semantic role labeling (SRL) \cite{gildeajurafsky2002}. In this task, we are given an input sentence, a target word that expresses a semantic predicate (typically a verb), and a semantic frame (i.e. a description of the predicate's possible semantic arguments). The goal is to label which other words in the sentence act as the predicate's arguments. For example, in the sentence ``IQ tests are a common method of identifying gifted children'', the predicate ``identifying'' can take multiple arguments, including ``Instrument'' and ``Target'', which are filled by ``IQ tests'' and ``gifted children'', respectively.  Understanding semantic roles is a fundamental challenge in NLP, and can be closely tied to question answering \cite{he2015qasrl}; for instance, understanding that IQ tests are the instrument of identification can answer the question ``What tools are used to identify gifted children?'' While semantic roles go beyond syntax, parse tree paths have been shown to be powerful features in SRL systems. In this work, we adapt their usage from natural to programming languages, and show that they can be used to infer semantic properties in programming languages as well.

%\TODO{Omer: I can also write another paragraph about syntactic paths (not necessarily PTPs) in other NLP applications.  Specifically,  one of the cooler applications is recognizing ``X is a Y'' relations (e.g.  ``many car manufacturers, including Ford and Toyota, ...''.  Having said that, the SRL example is very convincing IMHO.}

%Parse Tree Paths were first introduced by \citet{gildeajurafsky2002} for identifying semantic roles, filled by constituents of a natural language sentence within a semantic frame. Given an input sentence, a frame and a target word, the task is to label constituents in the sentence with their semantic roles. A target word is a word in the sentence, usually a verb, whose meaning represents the frame. A semantic frame is an abstract action or a relationship with participants. For example, a ``Statement'' frame contains semantic roles like ``Speaker'', ``Message'' and ``Addressee''. Many of the sets of semantic roles have been proposed by linguists, as part of grammatical theories describing the relationships between semantic roles and their syntactic position. Other sets have been proposed by computer scientists as part of NLP research. Labeling a sentence with semantic roles can be useful in information extraction from text, automatic question-answering systems, word-sense disambiguation, statistical machine translation and data mining.

%\citet{gildeajurafsky2002} also present statistical systems for automatically classifying semantic roles using human annotated boundaries, and for locating the boundaries of frame elements regardless of their correct label. These systems have integrated several types of features. While most of these features are specific to natural language and linguistics, Parse Tree Paths can be adapted to programming languages as well. %These systems have integrated 6 types of features:
%\begin{enumerate}
%\item Phrase type - the syntactic category of each phrase, such as $NP$, $PP$, etc.
%\item Governing Category - whether an element in the parse tree of the sentence is a descendant of a subject, or of an object of a verb.
%\item Parse Tree Path - as will be discussed in detail later in this section.
%\item Position - whether the element phrase occurs before or after the target word.
%\item Voice - whether the sentence is active or passive.
%\item Head Word - the syntactic head of the frame element, the word that determines the syntactic type of the phrase.
%\end{enumerate}

%\TODO{Omer: isn't this paragraph redundant given the intro?  If we want to keep it, some connection needs tobe made to fix the flow.}
%A Parse Tree Path is defined as the path from the target word through the parse tree to the constituent in question, represented as a continuous string of parse tree nonterminals, linked by symbols indicating upward or downward movement through the tree. The first element of the string is the part of speech of the target word, the last element is the phrase type of the constituent in question, and they are linked by the representation of the (only) path between them. Parse tree paths are particularly interesting because they encode the relationship between the syntactic and semantic aspects of elements.

%\TODO{Omer: Do we use any of these variants? If not, we can comment out this paragraph.}
%Since the introduction of Parse Tree Paths, a significant number of NLP systems have used these kinds of features for various types of NLP tasks. Several variations of the original paths have also been introduced, such as ``partial paths'', ``shallow paths'' and ``subpaths'' \cite{Johansson2005}. More recently, syntactic paths were used to capture word similarity via word2vec \cite{levy2014dependency}. \TODO{Omer: Would add the last sentence to a paragraph with other uses of syntactic paths.}

%Since programming languages are formal languages, their structural information is explicit, rich, and inherent. Even though natural language also has a structure, it tends to be less strict and more ambiguous. Therefore, a reasonable assumption is that using syntactic path features in programming languages can be even more advantageous than in natural languages.

\subsection{Conditional Random Fields}\seclabel{crfs}
%\para{Conditional Random Fields}
Probabilistic graphical models are a formalism for expressing the dependence structure of entities. Traditionally, graphical models have been used to represent the joint probability distribution $P\left(y,x\right)$, where \emph{y} represents an assignment of attributes for the entities that we wish to predict, and \emph{x} represents our observed knowledge about the entities~\cite{sutton2012, pearl2011bayesian, pearl2014probabilistic}. Such models are called \emph{generative} models. However, modeling the joint distribution requires modeling the marginal probability $P\left(x\right)$, which can be difficult, computationally expensive, and in our case requires us to estimate the distribution of programs~\cite{jsnice2015}.

A simpler solution is to model the conditional distribution $P\left(y|x\right)$ directly. Such models are called \emph{discriminative} models. This is the approach taken by \emph{Conditional Random Fields} (CRFs). A CRF is a conditional distribution $P\left(y|x\right)$ with an associated graphical structure~\cite{lafferty2001}. They have been used in several fields such as natural language processing, bioinformatics, and computer vision.

Formally, given a variable set $Y$ and a collection of subsets $\left\{ Y_{a}\right\} _{a=1}^{A}$ of $Y$, an \emph{undirected graphical model} is the set of all distributions that can be written as:
\begin{equation}
P\left(y\right)=\frac{1}{Z}\prod_{a=1}^{A}\Psi_{a}\left(y_{a}\right)
\end{equation}
where each $\Psi_{a}\left(y_{a}\right)$ represents a \emph{factor}. Each factor $\Psi_{a}\left(y_{a}\right)$ depends only on a subset $Y_{a}\subseteq Y$ of the variables. Its value is a non-negative scalar which can be thought of as a measure of how compatible the values $y_{a}$ are. The constant $Z$ is a normalization factor, also known as a partition function, that ensures that the distribution sums to $1$. It is defined as:
\begin{equation}
Z=\sum_{y}\prod_{a=1}^{A}\Psi_{a}\left(y_{a}\right)
\end{equation}

A CRF can also be represented as a bipartite undirected graph $G=\left(V,F,E\right)$, in which one set of nodes $V=\left\{ 1,2,...,\left|Y\right|\right\}$ represents indices of random variables, and the other set of nodes $F=\left\{ 1,2,...,A\right\}$  represents indices of the factors.

Several algorithms and heuristics were suggested for training CRFs and finding the assignment that yields the maximal probability~\cite{lafferty2001, koller2007, sutton2012}. We will not focus on them here, since our work is orthogonal to the learning model and the prediction algorithm.

Using CRFs to predict program properties was first proposed by~\citet{jsnice2015}, where each node represented an identifier in the code. These include variables, constants, function and property names. The factors represented the relationships or dependencies between those identifiers, and were \emph{defined by an explicit grammar and relations that were produced using semantic analysis}.

To demonstrate the use of AST paths with CRFs, we use CRFs exactly as they were used by~\citet{jsnice2015} but use AST paths instead of their original factors. Additionally, we introduce the use of unary factors (factors that depend on a single node). Unary factors are derived automatically by AST paths between different occurrences of the same program element throughout the program.

%\para{Training} After the graph, which is also referred to as a network, is obtained, training can be performed. Training, or learning, is a process of finding an optimal \emph{scoring} function. The scoring function consists of a set of weights, one for each combination of a factor and the attributes of the adjacent nodes. In other words, the scoring function maps tuples of $\left(attribute,relation,attribute\right)$ or $\left(relation,attribute\right)$ (in the unary case) to a positive real number. The score of the whole assignment is defined as the sum of the scores of its factors. We find the optimal set of weights such that desired assignments of predicted attributes \emph{y} get a higher score than other, less likely assignments. The goal in learning the weights is \emph{generalization}: the accurate prediction of the properties \emph{y} of any new program.

%\para{Prediction} After the model is trained, it is able to make structured predictions regarding properties of new sample programs, in a query referred to as \emph{maximum a posteriori} (MAP) inference. This query makes a joint prediction for all of the predicted attributes together, by optimizing the scoring function that was learned in the training phase, given the CRF of the input program. In this case, the nodes and the relations between them are given, as are some of the attributes of nodes (such as those that represent constants, or property names that we do not wish to infer), and the goal of the MAP inference is to find assignments of attributes for the rest of the nodes, such that the score of the entire assignment is maximal. The prediction objective is defined as finding:
%\begin{equation}
%y=\textrm{argmax}_{y'}P(y'|x)=\textrm{argmax}_{y'}score(y',x)
%\end{equation}
%In general, however, the problem is NP-hard, and heuristic techniques and approximations are usually used to find the assignment with the highest score\cite{koller2007}. We use Nice2Predict, which implements a greedy inference algorithm~\cite{jsnice2015}. Because the algorithm is greedy, it finds a local optimum and is not guaranteed to find the global optimum. However, it produces good results with a reasonable training time.

%As we find an optimal assignment, it contains the predicted names, and we can finally rename the identifiers in the input programs with the corresponding identifiers from the optimal assignment.

\subsection{Neural Word Embeddings}\seclabel{w2v}

Recently, neural-network based approaches have shown that syntactic and semantic properties of natural language words can be captured using low-dimensional vector representations, referred to as ``word embeddings'', such that similar words are assigned similar vectors~\cite{bengio2003,collobert2008,glove2014}. These representations are trained over large swaths of unlabeled text, such as Wikipedia or newswire corpora, and are essentially unsupervised. The produced vectors were shown to be effective for various NLP tasks~\cite{turian2010,collobert2011}.

In particular, the skip-gram model trained with the negative sampling objective (SGNS), introduced by~\citet{mikolovEfficient2013,mikolovDistributed2013}, has gained immense popularity via the word2vec toolkit, and substantially outperformed previous models while being efficient to train.
%The training objective of the skip-gram model is to find word vector representations that are useful for predicting the surrounding words in a sentence, by maximizing the probability:

SGNS works by first extracting the \emph{contexts}: $c_1, ..., c_n$ of each word $w$. It then learns a latent $d$-dimensional representation for each word and context in the vocabulary ($\vec{w}, \vec{c} \in \mathbb{R}^d$) by maximizing the similarity of each word $w$ and context $c$ that were observed together, while minimizing the similarity of $w$ with a randomly sampled context $c'$. In Mikolov et al.'s original implementation, each context $c_i$ is a neighbor of $w$, i.e., a word that appeared within a fixed-length window of tokens from $w$. \citet{levy2014dependency} extended this definition to include arbitrary types of contexts.

As shown by~\citet{levy2014neural}, this algorithm implicitly tries to encode the pointwise mutual information (PMI) between each word and context via their vector representations' inner products:
% (no space required between text and equation)
\begin{equation}
\vec{w}\cdot\vec{c} = PMI(w,c) = \log\frac{p(w,c)}{p(w)p(c)}
\label{Eq:skipgram}
\end{equation}
where each probability term models the frequency of observing a word $w$ and a context $c$ together (or independently) in the training corpus.


%One of the major contributions of word embeddings trained with SGNS (or other unsupervised methods) is that they allow supervised NLP systems to generalize to words that were not seen in the labeled training data (but do appear in the unlabeled corpus from which the embeddings were trained), and to some extent adapt to different domains. For example, if an SRL system was trained using labeled data from news articles, it might not generalize well to Wikipedia articles; however, incorporating word embeddings that were trained on a joint unlabeled corpus of news and Wikipedia articles could mitigate this problem. We leverage the same advantage for programming languages, and allow our algorithm to predict program properties across a variety of projects.

Recently, a simple model has achieved near state-of-the-art results for the lexical substitution task using embeddings that were learned by word2vec~\cite{melamud15}. The task requires identifying meaning-preserving substitutes for a target word in a given sentential context. The model in this work uses both word embeddings and context embeddings, and looks for a word out of the entire vocabulary whose embedding is the closest to all the given context embeddings and to the original word.
The similarities between the substitute word and each of the contexts and the original word are aggregated by an arithmetic mean or a geometric mean.

In contrast to natural language methods, our method does not use the original word but finds the unknown name by aggregating only the similarities between the candidate vector $w$ and each of the given context vectors $\widetilde{C}$:
\begin{equation}
prediction=argmax_{w\in W}\sum_{c\in \widetilde{C}}\left(w\cdot c\right)
\end{equation}

To demonstrate the use of AST paths with word2vec, we use AST paths as the context of prediction. As we show in~\secref{results}, using AST paths as context gives a relative improvement of $96\%$ over treating code as a token-stream and using the surrounding tokens as context.





==> featuregen - Copy/conclusion.tex <==
\section{Conclusion}
We presented a simple and general approach for learning from programs. The main idea is to represent a program using paths in its abstract syntax tree (AST). This allows a learning model to leverage the structured nature of source code rather than treating it as a flat sequence of tokens.

We show that this representation can be useful in a variety of programming languages and prediction tasks, and can improve the results of different learning algorithms without modifying the learning algorithm itself.

We believe that since the representation of programs using AST paths is fundamental to programming languages, it can be used in a variety of other machine learning tasks, including different applications and different learning models.


==> featuregen - Copy/evaluation.tex <==
\section{Evaluation}\seclabel{evaluation}

Since the goal of this work is to \emph{provide a representation of program elements}, we compared the effect of different representations on the accuracy of the learning algorithms.
To show that our approach can be applied to the representation of the input without modifying the learning algorithm, we used off-the-shelf learning algorithms but represented the input in each experiment using \emph{a different representation} (when possible).

Our evaluation aims to answer the following questions:
\begin{itemize}
\item How useful are AST paths compared to existing representations? (\secref{results})
\item How useful are AST paths across different programming languages, tasks and learning algorithms? (\secref{results})
\item Do AST paths just memorize the input, or do they capture deeper semantic regularities? (\secref{qualitative})
\item How long are the useful paths? How do the paths' length and width affect the results? (\secref{hyperparams})
\item How important is the concrete representation of paths? Which abstractions can be used to represent paths without reducing accuracy? (\secref{Abstractions})
\end{itemize}

\para{Leafwise and semi-paths}
Although the family of representations in this work includes n-wise paths and paths between any kind of AST nodes, for simplicity and feasible training time, we performed most of the experiments using leafwise-paths (paths between AST terminals) and semi-paths --- paths between an AST terminal and one of its ancestor nodes in the AST. The idea is that leafwise-paths are more diverse and therefore more expressive than semi-paths, but semi-paths provide more \emph{generalization}. Semi-paths allow us to generalize learning and capture common patterns in different programs, even if the full path does not recur.

An exception is the prediction of full types in Java, in which we predict types of expressions which are not necessarily terminals. In this case, we also used paths between terminals to the nonterminal in question.

\subsection{Prototype Implementation}\seclabel{implementation}

We implemented a cross-language tool called \tool. The tool consists of separate modules that parse and traverse the AST of a program in each different language, but the main algorithm is the same across all languages. Currently \tool contains modules for Java, JavaScript, Python and C\#, and it can be easily extended to any other language.

\para{AST construction and path extraction}
For Java we used~\citetalias{JavaParser}; for JavaScript we used~\citetalias{UglifyJS} for parsing and traversing the AST, along with additional modifications from~\citetalias{UnuglifyJS}; for Python we used the Python internal parser and AST visitor; and for C\# we used~\citetalias{Roslyn}.

\para{Learning algorithms} We experiment with two learning algorithms: Conditional Random Fields, based on the implementation of Nice2Predict~ \cite{jsnice2015}, and the word2vec based implementation of \citet{levy2014dependency}.

To support our representation in the learning engine side and produce a qualitative evaluation, we introduced minor extensions to the Nice2Predict framework:
\begin{itemize}
\item \emph{Support unary factors.} Previously, Nice2Predict supported only pairwise feature functions, and we implemented support for unary factors to express the relationship between different occurrences of the same identifier. Note that this is required because different AST nodes for the same identifier are merged into a single node in the CRF. Hence, a path between these nodes in the AST becomes a unary-factor in the CRF. This extension increases accuracy by about 1.5\%.
\item \emph{Top-k candidates suggestion.} CRFs output a single prediction for each program element. We implemented an additional API that receives a parameter $k$ and suggests the \emph{top-k} candidate names for each program element (this extension was adopted into Nice2Predict).
    This allowed us to manually investigate the quality of results (\secref{qualitative}). When all top-k predictions for a variable name captured similar notions, it increased our confidence that the model performs stable predictions.
\end{itemize}

\subsection{Experimental Setting}\seclabel{expsetting}

\para{Data sets}
For each language, we collected source code from public GitHub projects, and split it randomly to training, validation and test sets. Our data included the top ranked projects of each language and the projects that were forked the most. \tabref{datasets} shows the amount of data used for each language. Java required an order of magnitude more data than the other languages: we had to keep enlarging our Java dataset to achieve results that were close to the other languages.

Following recent work which found a large amount of code duplication in GitHub~\cite{dejavu2017}, we devoted much effort into filtering duplicates from our dataset, and especially the JavaScript dataset. To filter duplicates, we used file names, directory names (such as ``node\_modules''), and md5 of files. In Java and Python, which do not commit dependencies, duplication is less severe (as also observed by \citet{dejavu2017}). Furthermore, in our setting, we took the top-ranked and most popular projects, in which we observed duplication to be less of a problem (\citet{dejavu2017} measured duplication across \emph{all} the code in GitHub).

\para{Evaluation metric} For simplicity, in all the experiments we measured the percentage of exact match predictions, case-insensitive and ignoring differences in non-alphabetical characters. For example, this metric considers \scode{totalCount} as an exact match to \scode{total\_count}. An exception is the comparison to \citet{conv16}, who optimized their Java method name prediction model to maximize the F1 score over sub-tokens. In this case, we compared their model with ours on both exact match and F1 score. An unknown test label (``UNK'') was always counted as an incorrect prediction, or as a possibly partial prediction when using the F1 score, and our model never suggests ``UNK''. For example, if the true test label is \scode{get<UNK>}, our model could get partial precision and partial recall for predicting \scode{getFoo}.

\begin{table}[]
\centering
\footnotesize
\begin{tabular}{lrrrrrrr}
\toprule
                    & Total &\multicolumn{2}{c}{Training Set}  & \multicolumn{2}{c}{Test set} \\
Language            & repos & File   & Size (GB)    & File & Size (MB) \\ 
\midrule
Java                & $10,081$             & $1,717,016$        & $16$         & $50,000$        & 1001  \\ %\hline
JavaScript          & $6,863$             & $159,038$          & $3.4$        & $38,103$        & 130  \\ %\hline
Python              & $8,565$             & $458,771$          & $5.4$        & $39,941$         & 588 \\ %\hline
C\#                 & $1,000$             & $262,774$          & $4.7$        & $50,000$        & 1208   \\ 
\bottomrule
\end{tabular}
\caption{The amounts of data used for the experimental evaluation of each language.}
\tablabel{datasets}
\end{table}

\subsection{Quantitative Evaluation}\seclabel{results}

\input{results-table}
\input{results-nn-table}

We conducted several experiments to evaluate the usefulness of AST paths in different tasks and programming languages.
We performed the following quantitative experiments:
\begin{itemize}
	\item \emph{Prediction of variable names across all four languages}. Variable names have sufficient training data in all languages to produce meaningful results. In this experiment we used both CRFs and word2vec. As baselines we used the work of \citet{jsnice2015}, CRFs with token-based n-grams as factors, and a simple rule-based baseline. For JavaScript with word2vec, we used word2vec with linear token context as a baseline and show that path representations yield dramatic improvement.
	 	
	\item \emph{Prediction of method names across JavaScript, Java and Python}. We compared our general approach for method name prediction with \citet{conv16}, who used a convolutional neural network with attention.
%We note that in this experiment there is a difference in both input representation and learning algorithm between our suggested model and the baseline, although the training corpus is the same.

%who reports good results only while training and testing on disjoint parts of the \emph{same project}, and reports significantly worse results when training a single model that is usable across different projects.
	
	\item \emph{Prediction of full types in Java}. For Java, we compared our results to a synthetic (straw-man) baseline that predicts all types to be \scode{java.lang.String}. This baseline shows that despite the prevalence of the \scode{String} type, the task of type prediction is still very challenging. %As
\end{itemize}

In all of the following CRF experimental setups, ``no-path'' refers to a ``bag-of-words'' baseline, in which we used the same CRF learning algorithm, but used a single symbol to represent all relations. In this baseline, path information was hidden from the model during training and testing, and therefore it always assigned the same likelihood for each specific pair of identifiers, regardless of the syntactic relation between them. This baseline can be seen as a ``bag of near identifiers'' that uses the neighbors' names without their syntactic relation and therefore without considering the \emph{way} program elements are related.

\subsubsection{Predicting Variable Names}
To predict variable names, we used both CRFs and word2vec.

\para{Evaluation with CRFs} We present our evaluation results with CRFs for names in the top part of~\tabref{results}.
For JavaScript, where a tool that uses predefined features exists, we evaluated the other tool with the exact same datasets and settings, and the same AST terminals as CRF nodes, which makes the input representation (AST paths vs. their features) the only difference between the two experiments.
Using our representations yields $7.6\%$ higher accuracy than the previous work.

For Java, we compared the results with two baselines:
\begin{itemize}
\item \emph{CRFs $+$ n-grams} - this baseline uses the same CRF nodes as the path-based model, except that the relations between them are the \emph{sequential} n-grams. We chose $n=4$ as the value that maximizes accuracy on the validation set, such that the produced model consumes approximately the same amount of memory and disk as the path-based model.
\item \emph{Rule-based} - Since Java is a typed language which has a rich type system, and typical code tends to use a lot of classes and interfaces, we wonder whether the task of predicting variable names is easier in Java than in other languages and can be solved using traditional rule-based (non-learning) approaches. Our rule-based baseline predicts variable names based on the following pattern heuristics and statistics of the training corpus:
    \begin{itemize}
    \item \scode{for(int \underline{i} = ...) \{}
    \item \scode{this.<fieldName> = \underline{<fieldName>};}
    \item \scode{catch (... \underline{e}) \{}
    \item \scode{void set<fieldName>(... \underline{<fieldName>}) \{}
    \item Otherwise: use the type: \scode{HttpClient \underline{client}}.
    \end{itemize}
\end{itemize}

As shown, using CRFs with AST paths yields higher results than the baselines, in all the languages, showing that our representation yields higher results than manually defined features, n-grams, and rule-based approaches.
%We note that several prediction tasks for JavaScript and Python were examined by \citet{decisionTrees2016}. However, JavaScript name prediction was not evaluated, and name prediction in Python was examined and achieved a little lower accuracy (albeit with a different dataset).

\para{Evaluation with word2vec} We present our evaluation results with a word2vec based implementation in~\tabref{results-nn}. For comparison, we use two alternative approaches to represent the context for prediction:
\begin{itemize}
\item The \emph{linear token-stream} approach uses the surrounding tokens to predict a variable name. Surrounding tokens (e.g., values, keywords, parentheses, dots and brackets) may implicitly hint at the syntactic relations, without AST paths. This is the type of context usually used in NLP, in the original implementation of word2vec, and in many works in programming languages.
\item The \emph{path-neighbors, no-paths} approach uses the same surrounding AST nodes for contexts as AST paths, except that the path itself is hidden, and only the identity of the surrounding AST nodes is used. The goal of using this baseline is to show that the advantage of AST paths over token-stream is not only in their wider \emph{span}, but in the representation of the path itself.
\end{itemize}

Using word2vec with AST paths produces much better results compared to these baselines. This shows the advantage of using AST paths as context over token-stream based contexts, and the significance of using a representation of the paths for prediction.

\para{Limitations of evaluation}
We noticed that our models often predict names that are very similar but not identical to the original name, such as \scode{message} instead of \scode{msg}, or synonyms such as \scode{complete} instead of \scode{done}; these are counted as incorrect predictions. Moreover, we noticed that our models sometimes predict \emph{better} names than the original names. Therefore, the accuracy results are an underapproximation of the ability of AST paths to predict meaningful names.

Another limitation lies in the inability of CRFs and word2vec to predict out-of-vocabulary (OoV) names. As was previously observed~\cite{conv16, allamanis2015}, there are two main types of OoV names in programs: names that did not appear in the training corpus but can be composed of known names (neologisms), and entirely new names. The total OoV rate among our various datasets and tasks varied between $5-15\%$, and specifically $7\%$ for predicting variable names in JavaScript, and $13\%$ for Java method names. Several techniques were suggested to deal with each type of OoV~\cite{conv16, allamanis2015}, which we did not consider here and are out of scope of this work.

\para{Discussion} We note that the accuracy for Java is lower than for JavaScript. We have a few possible explanations:
\begin{inparaenum}[(i)]
	\item The JavaScript training set contains projects that are rather domain specific, mostly client and server code for web systems (for example, the terms \scode{request} and \scode{response} are widely used across all projects). In contrast, the Java code is much more varied in terms of domains.
	\item The Java naming scheme makes extensive use of compound names (e.g., \scode{multithreadedHttpConnectionManager}), and this is amplified by the type-based name suggestions for variables provided by modern Java IDEs. In contrast, the JavaScript variable names are typically shorter and are not an amalgamation of multiple words (e.g., \scode{value}, \scode{name}, \scode{elem}, \scode{data} are frequent names).
\end{inparaenum}

The accuracy of C\# is similar to Java, but using significantly less training data. We believe that C\# naming is more structured because the commonly used C\# IDE (VisualStudio), suggests variable names based on their types.

The accuracy for Python is lower than that of JavaScript. Manual examination of the training data shows that Python programs vary widely in code quality, making the training set more noisy than that of other languages. In addition, the variety of domains and IDEs for Python makes variable names less standard. Finally, Python is easy to write, even for non-programmers, and thus there is a wide variety of non-professional Python code. The low accuracy for Python is also consistent with \citet{decisionTrees2016}.

\para{Comparison of CRFs and word2vec}
We observe that the accuracy of \tool + CRFs is higher than that of \tool + word2vec, as can be seen in~\tabref{results}.
One reason is that, unlike CRFs, word2vec was not designed exactly for this prediction task. Originally, word2vec was intended to produce meaningful word embeddings: given a set of query path-contexts, the vectors of all of them are assigned the same weight for predicting the unknown value.

%Another reason is that given a set of query paths contexts and an unknown value, CRF uses candidates: it predicts only names that appeared with at least one of the query contexts in the training set, while word2vec can predict names out of the whole vocabulary, even if it appeared only with similar contexts, but never with any of the exact query paths.
Moreover, CRFs are relatively more interpretable. The weights assigned to each factor can be observed and explain a prediction posteriori.
However, word2vec was faster to train and much more memory efficient. In our evaluation, the memory required for training was over $200$GB for CRFs and only $10$GB with word2vec. Further, the training time of CRFs was up to $100$ hours, where word2vec required at most $5$ hours.

%A future work might design a custom neural network that is designed towards predicting an unknown value given a large set of contexts, and may give better results than both CRF and word2vec, while being as fast to train as word2vec and as interpretable as CRFs. This is out of the scope of this work, as this work is focused on representations of program elements rather than on the learning algorithms themselves.

The goal here is not to provide a fair comparison between CRFs and word2vec, as their prediction tasks are slightly different; our observations in this regard are merely anecdotal. The main goal is to compare \emph{different representations for the same learning algorithm} and show that each of the learning algorithms separately can be improved by plugging in our simple representation.

\subsubsection{Predicting Method Names}
We present our evaluation results for predicting method names in~\tabref{results}. Accuracy was similar for all languages ($\sim50\%$).

Good method names balance the need to describe the internal implementation of the method and its external usage~\cite{Host:2009:DMN:1615184.1615204}. For predicting method names, we use mostly the paths from within a method to its name, but when available in the same file, we also use paths from invocations of the method to the method name. Ideally, one would use paths from different files (and for library methods, even across projects), but this requires a non-local view, which we would like to avoid for efficiency reasons.

We use the internal paths from the leaf that represents the method name to other leaves within the method AST (which capture the method implementation) and the external paths from references of the method to their surrounding leaves (which represent the usage of the method). However, we observed that using only internal paths yields only $1\%$ lower accuracy.

In Java, CRFs with AST paths are compared to the model of \citet{conv16}, which we trained on the same training corpus. Since their model is optimized to maximize the F1 score over sub-tokens, \tabref{results} presents both exact accuracy and F1 score for method name prediction in Java. The table shows that CRFs with AST paths significantly improve over the previous work in both metrics.

\input{python_example}
\input{js_example}
\input{java_example}

\subsubsection{Predicting Full Types}
\begin{sloppypar}
Our results for predicting full types in Java using CRFs are shown in the bottom part of~\tabref{results}. Our goal is to predict the full type even when it explicitly appears in the code (e.g., \scode{com.mysql.jdbc.Connection}, rather than \scode{org.apache.http.Connection}). Here we also use paths from leaves to nonterminals which represent expressions. The evaluated types were only those that could be solved by a global type inference engine. Therefore, accuracy is the percent of correct predictions out of the results that are given by type inference.
\end{sloppypar}

Although a type inference engine still produces more accurate results than our learning approach, our results using AST paths are surprisingly good, especially considering the relative simplicity of our representation. We also note that type inference is a global task, and our approach reconstructs types locally without considering the global scope of the project.

CRFs with AST paths achieved $69.1\%$ accuracy when predicting full type for Java. We contrast this result with a na\"ive baseline that uniformly predicts the type \scode{java.lang.String} for all expressions. This naive baseline yields an accuracy of $24.1\%$, which shows the task is nontrivial, even when factoring out the most commonly used Java type.


\subsection{Qualitative Evaluation}\seclabel{qualitative}

Our qualitative evaluation includes:
\begin{itemize}
	\item An anecdotal study of name prediction in different languages. For JavaScript we also compared our predictions to those of \citet{jsnice2015} in interesting cases.
	\item An anecdotal study of top-k predictions for some examples, showing semantic similarities between predicted names as captured by the trained model.
\end{itemize}

\subsubsection{Prediction Examples}
\figref{pythonExample_p} shows an example of a Python program predicted using AST paths. It can be seen that all the names predicted using AST paths were renamed with meaningful names such as \scode{process}, \scode{cmd} and \scode{retcode}.

\begin{sloppypar}
\figref{jsExample} shows the default JavaScript example from {\small nice2predict.org}, predicted using AST paths and an online version of UnuglifyJS at {\small nice2predict.org}. We note that their online model was not trained on the same dataset as our model. The model which was trained using UnuglifyJS and our dataset yielded worse results. It can be seen that our model produced more meaningful names such as \scode{url} (instead of \scode{source}) and \scode{callback} (instead of \scode{n}).
\end{sloppypar}

\figref{javaExample} shows examples of Java programs. To demonstrate the expressiveness of AST paths, we deliberately selected challenging examples in which the prediction cannot be aided by the informative class and interface names that Java code usually contains (as in: \scode{HttpClient \underline{client}}). Instead, our model had to leverage the syntactic structure to predict the meaningful names: \scode{done}, \scode{values}, \scode{value} and \scode{count}.

\subsubsection{Semantic Similarity between Names}
%In this section we discuss a few interesting predictions that using AST paths has produced, compare them to the predictions of other approaches on the same examples, compare similar examples in different languages, and analyze the contribution of different paths in one of the examples.

\input{semsim-table}

It is interesting to observe the other \emph{candidates} that our trained model produces for program elements. As~\tabref{doneCandidates} shows, the next candidates after \scode{done} (in~\figref{code-example}) are: \scode{ended}, \scode{complete}, \scode{found}, \scode{finished}, \scode{stop} and \scode{end}, which are all semantically similar (in programs, not necessarily in natural language).
%
In many cases, AST paths capture the \emph{semantic similarity} between names, for example \scode{req}$\sim$\scode{request} and \scode{list}$\sim$\scode{array}, as shown in~\tabref{topk-similarities}. This supports our hypothesis that AST paths capture the semantic role of a program element.
%\para{Insensitivity to noise} Another interesting property of the \maxwidth parameter is the insensitivity to noise that a bigger width provides. Usually, functions that have similar usage of variables and methods have a similar general structure, but they are seldom exactly identical.


\subsection{Impact of Parameter Values}\seclabel{hyperparams}

In~\secref{application} we introduced and discussed the importance of the \maxlen and \maxwidth parameters. For each language we experimented with different combinations of values for \maxlen and \maxwidth on its validation set. We chose the values that produced the highest accuracy while still being computationally feasible when evaluating the model with the test set.

\para{Accuracy with different path length and width} We experimented with tuning the path parameters and observed their effect on the accuracy. The best parameter values for each prediction are shown in~\tabref{results}.

\input{accuracy-vs-len-figure}

For the task of name prediction, for all languages, the best path length is 6-7, and the best width is 3-4. The variations in path length stem from minor differences in the structure of the AST. For example, despite the similarity in source level between Java and C\#, the C\# AST is slightly more elaborate than the one we used for Java.

A drill-down of the accuracy given different parameter values for variable name prediction in JavaScript is shown in~\figref{accuracyvslength}. We observe that the \maxlen parameter has a significant positive effect, while the contribution of a larger \maxwidth is positive but minor. This observation affirms our initial hypothesis that our long-distance paths are fundamental and crucial to the accuracy of the prediction. It also confirms our belief that an automatic representation of code (rather than manually defined) is essential, since the long-distance paths are very unlikely to have been designed manually.

For the task of method name prediction, since there are significantly fewer paths, we could afford to set a high parameter value without too much tuning and still keep the training time and resources feasible. We therefore set the length in this case to $12$ for JavaScript, $10$ for Python, and just $6$ for Java.
%The size of the training set in Java is much larger, and to keep the total training time low without cutting the training set, we simply set a lower threshold for Java. We believe that with longer training time, the results for Java could be improved.

For the task of predicting full types in Java, we used length $4$ and width $1$, which yielded an accuracy of $69.1\%$. The intuition for the short path length is that in many cases the type of an expression can be inferred locally from other neighboring types, often from an explicit type declaration.

Higher values for \maxlen and \maxwidth resulted in higher training times, but combined with the \emph{downsampling} approach, it is possible to maintain a shorter training time while increasing the parameter values, and control the tradeoff between accuracy and training time.

\input{random-pigeon-figure}

\para{Downsampling} We wanted to measure the effect of training data size on accuracy and training time. Inspired by \citet{node2vec2016}, who used random walks to learn representations for neighborhoods of nodes in a network, we experimented with randomly omitting a fraction of the extracted path-contexts. After extracting path-contexts from all the programs in the training set, we randomly omitted each occurrence of a path-context in probability of $1-p$ (i.e., $p$ is the probability to keep it) and trained a model only on the remaining paths. As can be seen in~\figref{randompigeon}, randomly dropping contexts can significantly reduce training time, with a minimal effect on accuracy. %(the exact times are not presented here and significantly differ between different systems).
For example, for $p=0.8$ we observed exactly the same accuracy as for the complete set of paths ($p=1$), while training time was reduced by about $25\%$. Moreover, decreasing $p$ down to $0.2$ still yielded higher accuracy than UnuglifyJS but reduced training time by about $80\%$ (compared to $p=1.0$).

\subsection{Abstractions of AST Paths}\seclabel{Abstractions}
In order to evaluate the full expressiveness of AST paths, the previously reported experiments were performed using no abstraction, i.e. $\alpha_{id}$. However, it is also possible to use a higher level of abstraction. Instead of representing the whole path node-by-node with separating up and down arrows, it is possible to keep only parts of this representation. This abstraction results in less expressive paths and might represent two different paths as equal, but it enables decreasing the number of distinct paths, thus reducing the number of model parameters. Training will be faster as a result.

Different levels of path abstractions also allow us to evaluate the importance of different components of AST paths, or \emph{which components of AST paths contribute to their usefulness the most}. We experimented with several levels of abstraction:
\begin{itemize}
\item ``No-arrows'' - using the full path encoding, except the up and down symbols $\left\{\uparrow ,\downarrow\right\}$.
\item ``Forget-order'' - using paths without arrows and without order between the nodes: instead of treating a path as a \emph{sequence} of nodes, treat it as a \emph{bag} of nodes.
\item ``First-top-last'' - keeping only the first, top and last nodes of the path. The ``top'' node refers to the node that is hierarchically the highest, from which the direction of the path changes from upwards to downwards.
\item ``First-last'' - keeping only the first and last nodes.
\item ``Top'' - keeping only the top node.
\item ``No-paths'' - using no paths at all, and treating all relations between program elements as the same. The name of an element is predicted by using the bag of surrounding identifiers, without considering the syntactic relation to each of them.
\end{itemize}

All of the following experiments were performed using CRFs for variable names prediction, on the Java corpus and on the same hardware. In every experiment, the training corpus and the rest of the settings were identical. The number of training iterations was fixed.

\figref{abstractions_figure} shows the accuracy of each abstraction compared to the consumed training time. As shown, as more information is kept, accuracy is increased, with the cost of a longer training time. An interesting ``sweet-spot'' is ``first-top-last'', which reduces training time by half compared to the full representation, with accuracy that is as $95\%$ as good.

We also observe that the arrows and the order of the nodes in the path contribute about $1\%$ accuracy.

\input{abstractions_figure} 

==> featuregen - Copy/genericmacros.tex <==
%!TEX root=draft.tex

% Generic macros (nothing specific to this paper)

\usepackage{ifthen}
%
\newcommand{\todoi}[1]{}
%\newcommand{\todoi}[1]{}
\newcommand{\EYREM}[1]{{\color{red} \st{#1}}}
\newcommand{\EY}[1]{\TODO{EY:#1}}
\newcommand{\TODO}[1]{ {\color{blue} \bf #1} }
\newcommand{\DONE}[1]{ {\color{gray} \textbf{DONE - } #1} }
\newcommand{\OMIT}[1]{ {\color{gray} \bf #1} }
\newcommand{\AWK}[1]{ {\color{red} \bf #1} }
\newcommand{\TODOFN}[1]{ \footnote{{\bf #1}} }
\newcommand{\COMMENT}[1]{}
\newcommand{\ignore}[1]{}
\newcommand{\ie}{i.e.}
\newcommand{\eg}{e.g.}
%%% references definition
\newcommand{\lemref}[1]{Lemma~\ref{Lm:#1}}
\newcommand{\figref}[1]{Fig.~\ref{Fi:#1}}
\newcommand{\defref}[1]{Def.~\ref{Def:#1}}
\newcommand{\theref}[1]{Theorem~\ref{Th:#1}}
\newcommand{\tabref}[1]{Table~\ref{Ta:#1}}
\newcommand{\secref}[1]{Section~\ref{Sec:#1}}
\newcommand{\secrefs}[2]{Sections~\ref{Sec:#1}-\ref{Sec:#2}}
\newcommand{\ssecref}[1]{Sec.~\ref{Sec:#1}}
%\newcommand{\subref}[1]{Subsection~\ref{Sub:#1}}
\newcommand{\appref}[1]{Appendix~\ref{Se:#1}}
\newcommand{\exref}[1]{Example~\ref{Ex:#1}}
\newcommand{\algref}[1]{Algorithm~\ref{Alg:#1}}
\newcommand{\funcref}[1]{Function~\ref{Func:#1}}
\newcommand{\lnref}[1]{line~\ref{Ln:#1}}
\newcommand{\equref}[1]{Eq.~\ref{Eq:#1}}
\newcommand{\lemlabel}[1]{\label{Lm:#1}}
\newcommand{\figlabel}[1]{\label{Fi:#1}}
\newcommand{\deflabel}[1]{\label{Def:#1}}
\newcommand{\thelabel}[1]{\label{Th:#1}}
\newcommand{\tablabel}[1]{\label{Ta:#1}}
\newcommand{\seclabel}[1]{\label{Sec:#1}}
\newcommand{\sseclabel}[1]{\label{Sec:#1}}
%\newcommand{\sublabel}[1]{\label{Sub:#1}}
\newcommand{\applabel}[1]{\label{Se:#1}}
\newcommand{\exlabel}[1]{\label{Ex:#1}}
\newcommand{\alglabel}[1]{\label{Alg:#1}}
\newcommand{\funclabel}[1]{\label{Func:#1}}
\newcommand{\lnlabel}[1]{\label{Ln:#1}}
\newcommand{\equlabel}[1]{\label{Eq:#1}}

\theoremstyle{definition}
%\newtheorem{definition}{Definition}[]

%% TO Allow writing the TR in the same source
\newboolean{TR}
\setboolean{TR}{false}
\ifthenelse{\boolean{TR}}{
\newcommand{\TrSelect}[2]{#1}
\newcommand{\TrOnly}[1]{#1}
\newcommand{\SubOnly}[1]{}
\newcommand{\TrOnlyInFootnote}[1]{#1}
\newcommand{\TrOnlyInTable}[1]{#1}}
{
\newcommand{\TrSelect}[2]{#2}
\newcommand{\TrOnly}[1]{}
\newcommand{\SubOnly}[1]{#1}
\newcommand{\TrOnlyInFootnote}[1]{}
\newcommand{\TrOnlyInTable}[1]{}}

%% General macros
\newcommand{\Set}[1]{\{ \; {#1} \; \}}
\newcommand{\vbar}{\; | \;}
\newcommand{\notIn}{\not\in}
\newcommand{\sizeof}[1]{|{#1}|}
%% \newcommand{\isDefined}{=_{def}}
\newcommand{\isDefined}{\triangleq}

\newcommand{\lt}{$<$}
\newcommand{\gt}{$>$}

%% tminus: "thin minus", with less space around it;
%% telem: "thin element"
\newcommand{\tminus}{\!\! - \!\!}
\newcommand{\telem}{\! \in \!}

%% stexttt: "small" texttt
\newcommand{\stexttt}[1]{{\small \texttt{#1}}}

\newcommand{\mathify}[1]{\mathord{\mbox{#1}}}
\newcommand{\italMathId}[1]{\mathify{\textit{\textrm{#1}}}}
\newcommand{\romanMathId}[1]{\mathify{\textup{\textrm{#1}}}}
\newcommand{\ttMathId}[1]{\mathify{\textup{\texttt{#1}}}}

\newcommand{\ttsub}[2]{${\ttMathId{#1}}_{#2}$}
\newcommand{\ttsup}[2]{${\ttMathId{#1}}^{#2}$}
\newcommand{\mttsub}[2]{{\ttMathId{#1}}_{#2}}
\newcommand{\twoarray[2]}{\begin{array}{l}  #1 \\ #2 \end{array}}
\newcommand{\subsubsubsection}[1]{\emph{#1}:}




%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}

%\newenvironment{proof}[1][Proof]{\begin{trivlist}\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{definition}[1][Definition]{\begin{trivlist}\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{example}[1][Example]{\begin{trivlist}\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{remark}[1][Remark]{\begin{trivlist}\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

%\newcommand{\qed}{\nobreak \ifvmode \relax \else
%      \ifdim\lastskip<1.5em \hskip-\lastskip
%      \hskip1.5em plus0em minus0.5em \fi \nobreak
%      \vrule height0.75em width0.5em depth0.25em\fi}


==> featuregen - Copy/intro-ast-path.tex <==
\begin{figure}
\hspace{10mm}
\begin{subfigure}[b]{0.42\textwidth}
\lstset{language=JavaScript, basicstyle=\footnotesize\ttfamily,emph={fence},emphstyle=\underbar,escapeinside={(*@}{@*)}}
\begin{lstlisting}
while (!d) {
	if (someCondition()) {
		d = true;
	}
}
\end{lstlisting}
\caption{A simple JavaScript program.}
\label{Fi:code-example}
\end{subfigure}
%\hfill
\\
\begin{subfigure}[b]{0.42\textwidth}
\includegraphics[width=3in]{programPath_d}
\caption{The program's AST, and example to an AST path.}
\label{Fi:programPath}
\end{subfigure}
\caption{A JavaScript program and its AST, along with an example of one of the paths.}
\end{figure} 

==> featuregen - Copy/intro2.tex <==
\section{Introduction}\seclabel{Intro}

Leveraging machine learning models for predicting program properties such as variable names, method names, and expression types is a topic of much recent interest~\cite{jsnice2015,allamanis2015,conv16, decisionTrees2016, phog16, Maddison:2014:SGM:3044805.3044965}. These techniques are based on learning a statistical model from a large amount of code and using the model to make predictions in new programs. A major challenge in these techniques (and in many other machine-learning problems) is how to represent instances of the input space to facilitate learning~\cite{shwartz2014}. Designing a program representation that enables effective learning is a critical task that is \emph{often done manually for each task and programming language}.

\para{Our approach} We present a novel program representation for learning from programs. Our approach uses different path-based abstractions of the program's abstract syntax tree. This family of path-based representations is natural, general, fully automatic, and works well across different tasks and programming languages.

\para{AST paths} We define AST paths as paths between nodes in a program's abstract syntax tree (AST). To automatically generate paths, we first parse the program to produce an AST, and then extract paths between nodes in the tree. We represent a path in the AST as a sequence of nodes connected by up and down movements, and represent a program element as the set of paths that its occurrences participate in. \figref{code-example} shows an example JavaScript program. \figref{programPath} shows its AST, and one of the extracted paths. The path from the first occurrence of the variable \scode{d} to its second occurrence can be represented as:
{\small
\[
\textrm{SymbolRef }{\uparrow}\textrm{ UnaryPrefix! }{\uparrow}\textrm{ While }{\downarrow}\textrm{ If }{\downarrow}\textrm{ Assign= }{\downarrow}\textrm{ SymbolRef}
\]
}
This is an example of a pairwise path between leaves in the AST, but in general the family of path-based representations contains n-wise paths, which do not necessarily span between leaves and do not necessarily contain all the nodes in between. Specifically, we consider several choices of subsets of this family in~\secref{application}.

\input{intro-ast-path}

Using a path-based representation has several major advantages over existing methods:
\begin{enumerate}
\item Paths are generated automatically: there is no need for manual design of features aiming to capture potentially interesting relationships between program elements. This approach extracts unexpectedly useful paths, without the need for an expert to design features. The user is required only to choose a subset of our proposed family of path-based representations.
\item This representation is useful for any programming language, without the need to identify common patterns and nuances in each language.
\item The same representation is useful for a variety of prediction tasks, by using it with off-the-shelf learning algorithms or by simply replacing the representation of program elements in existing models (as we show in~\secref{results}).
%\item The features capture long distance syntactic relationships between program elements, and may thus provide rich context for making a prediction.
\item AST paths are purely syntactic, and do not require any semantic analysis.
%\item The method is local, and works on a small code fragment as a single function, without requiring additional dependencies from the whole project as input.
\end{enumerate}

%Our work is inspired by \emph{Parse Tree Paths} in NLP, where these paths, which are syntactic in nature, are used to infer the \emph{semantic} relations between elements in a sentence \cite{gildeajurafsky2002}. In NLP, a \emph{path-feature} is defined as the path from a word in the sentence, called the \emph{target word}, through the parse tree, to another word or constituent that we wish to label. Paths are used with other features to train various types of semantic role labeling classifiers, as we outline in~\secref{nlp}.
%\added[id=mz]{Parse Tree Paths in Natural Language are different from those we extract from programs, as we describe in more detail in \secref{ExtractingPaths}.}
%More recently, syntactic paths were used to capture word similarity via word2vec \cite{levy2014dependency}. Uri: it's not critical for the intro, we mention and cite this paper in the background section

\paragraph{Tasks} In this paper, we demonstrate the power and generality of AST paths on the following tasks:
\begin{itemize}
\item \textbf{Predicting names for program elements} Descriptive and informative names for program elements such as variables and classes play a significant role in the readability and comprehensibility of code. Empirical studies have shown that choosing appropriate names makes code more understandable~\cite{takang96}, reduces code maintenance efforts, and leads to fewer bugs~\citep{butler2009}. A study in the Psychology of Programming suggests that the ways in which programmers choose names reflect deep cognitive and linguistic influences~\cite{liblit2006}. A meaningful name describes the role of a program element, carries its semantic meanings, and indicates its usage and behavior throughout the program.
\item \textbf{Predicting method names} Good method names adequately balance the need to describe the internal implementation of the method and its external usage~\cite{Host:2009:DMN:1615184.1615204}. When published in a popular library's API, descriptive and intuitive method names facilitate the use of methods and classes, while poorly chosen names can doom a project to irrelevance~\cite{allamanis2015}. Although method names are clearly program elements and can be predicted by the previous task, in this task we assumes that all the other names in the method are given, along with the names of the elements around the method invocation, when available in the same file.
\item \textbf{Predicting expression types} Statistical type prediction allows (likely) types of expressions to be inferred without the need for type inference, which often requires a global program view (possibly unavailable, e.g., in the case of snippets from sites such as StackOverflow). %\TODO{Omer: is this a new task? Do you provide a new dataset? If so, it should be stated as part of the novelty claim. Otherwise, citations are needed.}
\end{itemize}


%The extracted paths are used as representations of program elements in machine learning models, which are trained to predict method names, variable names and types, using different learning algorithms, and for different programming languages.

\begin{figure*}
\centering
\includegraphics[width=7in]{overview-snip2}
%\caption{The partial AST of the statement.}
\caption{An overview of our approach. We start with a code snippet $\mathcal{C}$, and extract its path representation to be used as an input to machine learning models. The AST and paths were extracted from the example program in~\figref{code-example}.}
\label{Fi:overview_fig}
\end{figure*}

\citet{jsnice2015} used relations in the AST as features for learning tasks over programs. They defined an explicit grammar to derive features which capture specific relationships between nodes in the AST of JavaScript programs, as well as relations produced by language-specific semantic analysis, such as ``may call'' and ``may access''. We show that our \emph{automatic general representation} performs better than their features for their original task, and also generalizes to drive two different learning algorithms and three different prediction tasks, over different programming languages.

Paths in an AST have also been used by~\citet{phog16} and by~\citet{decisionTrees2016,raychev2016noisy} for a different goal: identifying context nodes. These works do not use the paths themselves as a representation of the input, and the prediction is only affected by the context node that was found on the other end of the path.  In our work, we use the path itself as a representation of a program element. Therefore, the prediction depends not only on the context node but also on \emph{the way it is related} to the element in question.

\citet{allamanis2015} defined the challenging task of predicting method names, which can be viewed as a form of function summarization~\cite{conv16}. We show that our representation performs better by being able to learn across projects.
	
We provide a more elaborate discussion of related work, including deep learning approaches, in~\secref{relatedWork}.

\para{Contributions} The main contributions of this paper are:
\begin{itemize}
\item A new, general family of representations for program elements. The main idea is to use AST paths as representations of code.
\item A cross-language tool called \tool, which is an implementation of our approach for predicting program element names, method names, and types.
\item An evaluation on real-world programs. Our experiments show that our approach produces accurate results for different languages (JavaScript, Java, Python, C\#), tasks (predicting variable names, method names, types) and learning algorithms (CRFs, word2vec). Furthermore, for JavaScript and Java, where previous methods exist, our automatic approach produces more accurate results.
\end{itemize}



==> featuregen - Copy/java_example.tex <==
\begin{figure*}[]
\centering
\begin{tabular}{|l|l|}
\hline
Stripped names & AST paths + CRFs \\ \hline

\begin{subfigure}[b]{0.33\textwidth}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (a){
\lstset{language=Java, basicstyle=\scriptsize\ttfamily,emphstyle=\underbar,escapeinside={(*}{*)}}

\begin{lstlisting}
boolean (*\bfseries d*) = false;
while (!(*\bfseries d*)) {
    if (someCondition()) {
        (*\bfseries d*) = true;
    }
}
\end{lstlisting}};
%\caption{}
%\label{Fi:minifiedWhileJava}
\end{subfigure}
         &
         \begin{subfigure}[b]{0.39\textwidth}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (b){
\lstset{language=Java, basicstyle=\scriptsize\ttfamily,emphstyle=\underbar,escapeinside={(*}{*)}}

\begin{lstlisting}
boolean (*\bfseries done*) = false;
while (!(*\bfseries done*)) {
    if (someCondition()) {
        (*\bfseries done*) = true;
    }
}
\end{lstlisting}};
%\caption{}
%\label{Fi:ourWhileJava}
\end{subfigure}
\\ \hline
\begin{subfigure}[b]{0.33\textwidth}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (c){
\lstset{language=Java, basicstyle=\scriptsize\ttfamily,emphstyle=\underbar,escapeinside={(*}{*)}}

\begin{lstlisting}
int count(List<Integer> (*\bfseries x*), int (*\bfseries t*)) {
    int (*\bfseries c*) = 0;
    for (int (*\bfseries r*): (*\bfseries x*)) {
        if ((*\bfseries r*) == (*\bfseries t*)) {
            (*\bfseries c*)++;
        }
    }
    return (*\bfseries c*);
}
\end{lstlisting}};
%\caption{}
%\label{Fi:minifiedCountJava}
\end{subfigure}
         &
         \begin{subfigure}[b]{0.39\textwidth}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (d){
\lstset{language=Java, basicstyle=\scriptsize\ttfamily,emphstyle=\underbar,escapeinside={(*}{*)}}
\begin{lstlisting}
int count(List<Integer> (*\bfseries values*), int (*\bfseries value*)) {
    int (*\bfseries count*) = 0;
    for (int (*\bfseries v*): (*\bfseries values*)) {
        if ((*\bfseries v*) == (*\bfseries value*)) {
            (*\bfseries count*)++;
        }
    }
    return (*\bfseries count*);
}
\end{lstlisting}};
%\caption{}
%\label{Fi:ourCountJava}
\end{subfigure}
\\ \hline
\end{tabular}
\caption{Examples of Java programs with stripped names and with predictions produced using our AST paths. We deliberately selected challenging examples in which the prediction cannot be aided by specific classes and interfaces.}
\figlabel{javaExample}
\end{figure*}

==> featuregen - Copy/js_example.tex <==
\begin{figure*}[]
\centering
\begin{tabular}{|l|l|l|}
\hline
Stripped Names & AST Paths + CRFs & \url{nice2predict.org}  \\ \hline
\begin{subfigure}[b]{0.3\textwidth}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (e){
\lstset{language=JavaScript, basicstyle=\scriptsize\ttfamily,emphstyle=\underbar,escapeinside={(*}{*)}}
\begin{lstlisting}
function f((*\bfseries a*), (*\bfseries b*), (*\bfseries c*)) {
  (*\bfseries b*).open('GET', (*\bfseries a*), false);
  (*\bfseries b*).send((*\bfseries c*));
}
\end{lstlisting}};
%\caption{}
%\label{Fi:minifiedRequest}
\end{subfigure}
&
\begin{subfigure}[b]{0.3\textwidth}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (f){
\lstset{language=JavaScript, basicstyle=\scriptsize\ttfamily,emphstyle=\underbar,escapeinside={(*}{*)}}

\begin{lstlisting}
function f((*\bfseries url*), (*\bfseries request*), (*\bfseries callback*)) {
  (*\bfseries request*).open('GET', (*\bfseries url*), false);
  (*\bfseries request*).send((*\bfseries callback*));
}
\end{lstlisting}};
%\caption{}
%\label{Fi:ourRequest}
\end{subfigure}
&
\begin{subfigure}[b]{0.3\textwidth}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (i){
\lstset{language=JavaScript, basicstyle=\scriptsize\ttfamily,emphstyle=\underbar,escapeinside={(*}{*)}}

\begin{lstlisting}
function f((*\bfseries source*), (*\bfseries req*), (*\bfseries n*)) {
  (*\bfseries req*).open("GET", (*\bfseries source*), false);
  (*\bfseries req*).send((*\bfseries n*));
}
\end{lstlisting}};
%\caption{}
%\label{Fi:unuglifyRequest}
\end{subfigure}            \\ \hline
\end{tabular}
\caption{Example of a JavaScript program with stripped names, with predictions produced using our AST paths and an online version of UnuglifyJS at {\small nice2predict.org}. This is the default example shown at {\small nice2predict.org}.}
\figlabel{jsExample}
%\tikz[remember picture,overlay]\draw[line width=3mm,-latex,gray] ([yshift=-4mm, xshift=45mm]a.west) --node[right = 3mm,black]{} ([yshift=-4mm]b.west);
%\tikz[remember picture,overlay]\draw[line width=3mm,-latex,gray] ([yshift=-4mm, xshift=45mm]c.west) --node[right = 3mm,black]{} ([yshift=-4mm]d.west);
%\tikz[remember picture,overlay]\draw[line width=3mm,-latex,gray] ([yshift=-4mm, xshift=45mm]e.west) --node[right = 3mm,black]{} ([yshift=-4mm]f.west);
\end{figure*} 

==> featuregen - Copy/overview-figure.tex <==
\begin{figure*}
\centering
\begin{minipage}{7in}
\hspace{0.6in}
\begin{tabular}{ccc}
\begin{subfigure}[b]{0.5\textwidth}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (a){
\lstset{language=JavaScript, basicstyle=\footnotesize\ttfamily,emphstyle=\underbar,escapeinside={(*}{*)}}

\begin{lstlisting}
while (!(*\bfseries d*)) {
	if (someCondition()) {
		(*\bfseries d*) = true;
	}
}
\end{lstlisting}};
\caption{}
\figlabel{minifiedWhileOverview}
\end{subfigure}

&	
&
\hspace*{-2cm}
\begin{subfigure}[b]{0.5\textwidth}
\addtocounter{subfigure}{3}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (e){
\lstset{language=JavaScript, basicstyle=\footnotesize\ttfamily,emphstyle=\underbar,escapeinside={(*}{*)}}

\begin{lstlisting}
while (!(*\bfseries done*)) {
	if (someCondition()) {
		(*\bfseries done*) = true;
	}
}
\end{lstlisting}};
\caption{}
\label{Fi:renamedWhile}
\end{subfigure}
\\
\\
\begin{subfigure}[a]{0.5\textwidth}
\addtocounter{subfigure}{-4}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (b){\includegraphics[width=.7\linewidth, clip=true]{whileMinifiedPath}};
%\includegraphics[]{whileMinifiedPath}
\caption{}
\label{Fi:treeWhile}
\end{subfigure}
&
&
\hspace*{-2cm}
\begin{subfigure}[a]{0.5\textwidth}
\addtocounter{subfigure}{1}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (d){\includegraphics[width=.7\linewidth,clip=true]{whileCRF-word2vec}};
%\includegraphics[]{whileCRF}
\caption{}
\label{Fi:crfWhile}
\end{subfigure}
\\
\\
\\
\\
\multicolumn{3}{c}{
\begin{subfigure}[]{1\textwidth}
\scriptsize
\addtocounter{subfigure}{-2}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (c){
\begin{tabular}{@{}llll@{}}
\toprule
Identifier & Path                                                                                                                                                                       & Identifier \\ \midrule
\textbf{d}        & \textbf{SymbolRef$\uparrow$UnaryPrefix!$\uparrow$While$\downarrow$If$\downarrow$Call$\downarrow$SymbolRef}                                                                                                                                             & \textbf{someCondition}\\ \midrule
\textbf{d}        & \textbf{SymbolRef$\uparrow$UnaryPrefix!$\uparrow$While$\downarrow$If$\downarrow$Statement$\downarrow$Assign=$\downarrow$SymbolRef}~~~~~~~~~~~~~~~~~~~~~                                                                                                                                   & \textbf{d}\\ \midrule
\textbf{d}        & \textbf{SymbolRef$\uparrow$UnaryPrefix!$\uparrow$While$\downarrow$If$\downarrow$Statement$\downarrow$Assign=$\downarrow$True}                                                                                                                                             & \textbf{true}\\ \midrule
\textbf{someCondition}        & \textbf{SymbolRef$\uparrow$Call$\uparrow$If$\downarrow$Statement$\downarrow$Assign=$\downarrow$SymbolRef}                                                                                                                                             & \textbf{d}\\ \midrule
\textbf{d}        & \textbf{SymbolRef$\uparrow$Assign=$\downarrow$True}                                                                                                                                             & \textbf{true}\\ \midrule
\end{tabular}
};
%\includegraphics[]{whileMinifiedPath}
\caption{}
\tablabel{tableWhile}
\end{subfigure}
}

\end{tabular}

\tikz[remember picture,overlay]\draw[line width=2mm,-latex,gray] ([xshift=-10mm, yshift=6mm]a.south -| b.north) --node[right = 2mm,black] {\small Parse program} ([xshift=-10mm]b.north);
\tikz[remember picture,overlay]\draw[line width=2mm,-latex,gray] ([xshift=-36mm]b.south -| c.north) -- node[right = 2mm,black] {\small Extract paths} ([xshift=-36mm, yshift = 2mm]c.north);
\tikz[remember picture,overlay]\draw[line width=2mm,-latex,gray] ([xshift=-10mm, yshift = 2mm]c.north -| d.south) -- node[right = 2mm,black] {\small Learning algorithm} ([xshift=-10mm]d.south);
\tikz[remember picture,overlay]\draw[line width=2mm,-latex,gray] (d.north -| e.south) -- node[right = 2mm,black] {\small Predict} ([yshift=5mm]e.south);
\caption{An overview of the use of AST paths in learning models. A simple program (a) is parsed to construct the AST (b), from which AST paths (c) are extracted. Different learning algorithms (CRF, word2vec) can be used (d) to predict program properties. In the resulting program (e), the predicted name for \scode{d} is \scode{done}.}
\end{minipage}
\end{figure*} 

==> featuregen - Copy/overview.tex <==
\section{Overview}\label{Se:Overview}

In this section, we illustrate our approach with a simple JavaScript program for the task of predicting names; as we show in later sections, the same approach also applies to other tasks, other languages, and other learning algorithms.

Given a program with non-descriptive names, our goal is to predict likely names for local variables and function parameters. The non-descriptive names could have been given by an inexperienced programmer, or could have been the result of deliberate stripping. In the latter case, we refer to such a program as a program with \emph{stripped names}. Stripping names can be part of a minification process in JavaScript, or obfuscation in Java and other languages.

%\input{overview-figure}


Consider the code snippet of~\figref{code-example}. This simple snippet captures a common programming pattern in many languages. Suppose that we wish to find a better name for the variable \scode{d}.

\para{Program element representation} The main idea of our approach is to extract paths from the program's AST and use them to represent an element, such as the variable \scode{d}, in a machine learning model. \figref{overview_fig} shows an overview of this process.
First, we parse the query program to construct an AST. Then, we traverse the tree and extract paths between AST nodes. To simplify presentation, in this example we only consider pairwise paths between AST leaves. We assume that a path is represented as a sequence of AST nodes, linked by up and down movements (denoted by arrows). As we describe in~\ssecref{application}, the path can also connect a leaf and a higher nonterminal in the AST, connect several nodes (n-wise path), and can be abstracted in different levels.

Consider the $p_{1}$ in~\figref{overview_fig}, between the two  occurrences of the variable \scode{d}:
\begin{equation}
\footnotesize
\textrm{SymbolRef }{\uparrow}\textrm{ UnaryPrefix! }{\uparrow}\textrm{ While }{\downarrow}\textrm{ If }{\downarrow}\textrm{ Assign= }{\downarrow}\textrm{ SymbolRef}
\tag{I}\label{eq:dTodPath}
\end{equation}
The path expresses the fact that the variable \scode{d} is used, with negation, as a stopping condition of a ``while'' loop, and then assigned a new value if an ``if'' condition inside the loop evaluates to \scode{true}. This path alone expresses the fact that \scode{d} is the stopping condition of the loop. %: when its value is \scode{true} the ``while'' loop stops, and its value is changed when the ``if'' condition is met.

The path $p_{4}$ in~\figref{overview_fig}, between the variable \scode{d} and the value \scode{true} is:
\begin{equation}
\footnotesize
\textrm{SymbolRef }{\uparrow}\textrm{ Assign= }{\downarrow}\textrm{True}
\tag{II}\label{eq:dToTruePath}
\end{equation}
This path captures the fact that the assignment changes the value of \scode{d} to \scode{true}, and therefore it is indeed the assignment that stops the loop.

\para{Prediction}
By observing these two paths, a programmer is likely to name \scode{d} ``done'', ``complete'', ``stop'' or something similar. Indeed, a learning model that was trained using our representation predicts that the most likely name for the variable is \scode{done}, and neither ``done'', ``complete'', nor any similar name was predicted by past work %\citetalias{UnuglifyJS} (\figref{unuglifyWhile}) or \citetalias{JSNice}
for this example. %Other examples comparing the models are shown in~\figref{jsExamples}.

\para{Learning algorithms}
The learning model can vary between different algorithms, presenting tradeoffs of efficiency and accuracy. In~\secref{results} we show that both CRFs and word2vec can be used for this prediction task.
%We show that prediction using word2vec produces less accurate results, but with significantly lower memory requirements.
In both of these learning algorithms, using AST paths produces better results than the alternative representations, whether they are manually designed or sequence-based representations.

\para{Path abstractions} Automatic generation may produce a prohibitively large number of paths. To control the number of paths, \emph{higher levels of abstraction} can be used. Instead of representing the whole path node-by-node, it can be further abstracted by keeping only parts of it, which results in similar paths being represented equally, as we show in~\secref{Abstractions}. Another way to control the number of paths is to limit the number of extracted paths. We provide hyper-parameters (i.e., model configurations that are not tuned by the optimization process) that control the maximal length and width of AST paths.
The number of extracted paths can be further reduced using downsampling, with minimal impact on accuracy and a significant saving in training time (\ssecref{results}). These methods make the accuracy -- training time tradeoff tunable.

\begin{figure}[]
\begin{subfigure}[t]{0.25\textwidth}
\lstset{language=JavaScript, basicstyle=\footnotesize\ttfamily,emphstyle=\underbar,escapeinside={(*}{*)}}
\begin{lstlisting}
var (*\bfseries d*) = false;
while(!(*\bfseries d*)) {
    doSomething();
    if (someCondition()) {
        (*\bfseries d*) = true;
    }
}
\end{lstlisting}
\caption{}
\figlabel{fullDone}
\end{subfigure}%
\unskip \vrule
\hspace{3mm}
\begin{subfigure}[t]{0.2\textwidth}
\lstset{language=JavaScript, basicstyle=\footnotesize\ttfamily,emphstyle=\underbar,showlines=true,escapeinside={(*}{*)}}
\begin{lstlisting}

someCondition();
doSomething();
var (*\bfseries d*) = false;
(*\bfseries d*) = true;


\end{lstlisting}
\caption{}
\figlabel{indistinguishableDone}
\end{subfigure}
\caption{An example for two code snippets that are indistinguishable by the model of~\citet{jsnice2015}, and are easily distinguishable by AST paths.}
\figlabel{similarWhile}
\end{figure}

\para{The discriminative power of AST paths} Examples indistinguishable by manually designed representations will always exist. For example, \citetalias{UnuglifyJS}~\cite{jsnice2015} extracts an identical set of relations (and therefore predicts the same name for \scode{d}) for the example in~\figref{fullDone} and for the simplified example in~\figref{indistinguishableDone}, even though the variable \scode{d} clearly does not play a similar role in these two examples. In contrast, these two examples are easily distinguishable using our AST paths.

%\para{Prediction} We group the ends of the paths by identifiers that refer to the same program element, and construct the CRF with a node for each program element and a factor for each path, as can be seen in \figref{crfWhile}. The CRF contains pairwise factors that represent paths between different program elements; it also contains one unary factor that represents path \ref{eq:dTodPath} between the variable \scode{d} and its other occurrence. When the CRF is constructed, we perform MAP inference, as will be described in \secref{crfs}, using a statistical model that was trained on paths from the training data. Finally, the elements in the original program can be renamed to the predicted names, as shown in \figref{renamedWhile}.

\para{Key aspects} The example highlights several key aspects of our approach:
\begin{itemize}
\item Useful paths such as path~\ref{eq:dTodPath} span multiple lines of the program, but are also supported by shorter paths like path~\ref{eq:dToTruePath}, which only spans a single program line. Short paths alone are not enough to predict a meaningful name. Making a prediction using all paths that an element participates in provides a rich context for predicting the name of the element.
%\item It is very unlikely that a path such as path~\ref{eq:dTodPath} could have been designed manually as a feature. The number of potentially useful paths is huge, and no expert could have thought of all possible paths.
\item No special assumptions regarding the AST or the programming language were made, making the same mechanism useful in other languages in a similar way. %In \secref{evaluation}, we present results for JavaScript, Java, Python and C\#.
\item This representation can be plugged into existing models as a richer representation of the input code, without interfering with the learning algorithm itself. %In \secref{evaluation}, we present results using both CRF and word2vec.
\item AST paths can distinguish between programs that previous works could not.
\item In addition to predicting \scode{done}, a model trained with AST paths can propose several semantically similar names, as we demonstrate in~\ssecref{results}. This shows that AST paths are strong indicators of the program element's semantics.
\end{itemize}



==> featuregen - Copy/python_example.tex <==
\begin{figure*}[]
\centering
\begin{tabular}{|l|l|}
\hline
Stripped names & AST paths + CRFs \\ \hline
\begin{subfigure}[b]{0.33\textwidth}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (a){
\lstset{language=Java, basicstyle=\scriptsize\ttfamily,emph={c,p,o,e,r},emphstyle=\bfseries,escapeinside={(*}{*)},morekeywords={def,for,in}}
\begin{lstlisting}
def sh3(c):
    p = Popen(c, stdout=PIPE,
        stderr=PIPE, shell=True)
    o, e = p.communicate()
    r = p.returncode
    if r:
        raise CalledProcessError(r, c)
    else:
        return o.rstrip(), e.rstrip()
\end{lstlisting}};
\end{subfigure}
         &
\begin{subfigure}[b]{0.39\textwidth}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (b){
\lstset{language=Java, basicstyle=\scriptsize\ttfamily,emph={cmd,process,out,err,retcode},emphstyle=\bfseries,escapeinside={(*}{*)},morekeywords={def,for,in}}

\begin{lstlisting}
def sh3(cmd):
    process = Popen(cmd, stdout=PIPE,
        stderr=PIPE, shell=True)
    out, err = process.communicate()
    retcode = process.returncode
    if retcode:
        raise CalledProcessError(retcode, cmd)
    else:
        return out.rstrip(), err.rstrip()
\end{lstlisting}};
\end{subfigure}
\\ \hline
\end{tabular}
\caption{Example of a Python program with stripped names and with predictions produced using our AST paths.}
\label{Fi:pythonExample_p}
\end{figure*} 

==> featuregen - Copy/relatedWork.tex <==
\section{Related Work}\seclabel{relatedWork}

\para{Naming in Software Engineering} Several studies about naming in code have been conducted \cite{takang96, butler2009, Host:2009:DMN:1615184.1615204,allamanis2015}.
%A technique for inferring naming rules for methods has been developed in \cite{Host:2009:DMN:1615184.1615204}. Using these rules, ``naming bugs'' can be identified.
%, and more suitable names can be suggested
%This work is specifically tailored to Java code,
%This work uses rules that depend on attributes that were manually crafted for Java, while our approach does not require manual definition of rules or features for different languages.
%Another approach
%Another work has used an NLP technique of part-of-speech (POS) tagging for programming languages purposes \cite{Binkley:2011:III:1985441.1985471}. This work has used a POS tagger on field names, to tag names with POS tags such as ``noun'' and ``verb''. Based on these tags, rules were manually identified, could be checked on new input programs, and violations could be detected, suggesting that the field name is inadequate. This approach was only shown to detect naming violations, but not to suggest new, better names. In contrast to our approach, the detection rules in this work were manually identified, and therefore the method could not be applied to other programming languages without identifying new rules.
Some of them applied neural network approaches for various applications.
An approach for inferring method and class names was suggested by \citet{allamanis2015}, by learning the similarity between names; however, they used features that were manually designed for a given task.
A recent work presents a convolutional attention model \cite{conv16} and evaluates it by predicting method names. In \secref{evaluation}, we show that using our general approach yields better results.

Several works have studied the use of NLP techniques in programming languages, for applications such as estimating code similarity \cite{Zilberstein:2016:LCN:2986012.2986013}, naming convention recommendations \cite{Allamanis:2014:LNC:2635868.2635883}, program synthesis \cite{Desai:2016:PSU:2884781.2884786}, translation between programming languages \cite{Karaivanov:2014:PST:2661136.2661148} and code completion \cite{raychev14, Hindle:2012:NS:2337223.2337322, Maddison:2014:SGM:3044805.3044965}. A bimodal modeling of code and natural language was suggested by \citet{bimodal15}, for tasks of code retrieval given a natural language query, and generating a natural language description given a code snippet.


A recent work presented a model that uses LSTM for code summarization, which is interpreted as generating a natural language description for given program~\cite{codenn16}. This work presents impressive results, but requires a very large amount of human-annotated data.


\ignore{
A previous work reduced the problem of code completion to NLP by using the n-gram model \cite{raychev14}. An n-gram model has also been used by \citet{Allamanis:2014:LNC:2635868.2635883} to develop a naming convention recommendation tool.
The tool trains over a specific codebase, and learns this codebase's coding conventions by learning an n-gram model over tokens, rather than words.
However, while code conventions are project-specific, our representation can be used in both project-specific and cross-project models.
}
%According to this model, the probability of the next word to appear depends on the identity of the \emph{n-1} words preceding the predicted position.
%To demonstrate the approach, a code-completion tool was created, that uses a statistical language model to compute a set of completion candidates for ``holes'' in a given program.
%The main difference from our approach is that this work treats a program as a \emph{sequence} of words rather than a \emph{tree}, and without considering the solid and unambiguous structure of programs as compared to natural language sentences.
%Then, the model can be used to fix existing conventions violations. The tool has automatically generated patches for popular open-source projects.
%However, because coding conventions are project-specific, and tend to evolve during a project's lifetime, this tool is at a disadvantage in the early stages of a project.
%Our approach differs in the universality of its recommendations.



\para{Predicting program properties using probabilistic graphical models} CRFs have been used for structured prediction of program properties in JavaScript and Android Java code \cite{jsnice2015, android2016}. The method has been shown to produce good results for prediction of names and types, by modeling programs with CRFs. \citet{jsnice2015} defined relationships between program elements using an explicit grammar specific to JavaScript. The possible relationships span only a single statement, and do not include relationships that involve conditional statements or loops. \citet{android2016} also defined several types of features and the conditions in which each of them is used. These works motivate a representation that is extractable automatically and can be applied to different languages. Instead of defining the relationships between program elements in advance, we learn them from the training data, in an automatic process that is similar for different languages. %As we show in \secref{evaluation}, automatic generation of AST paths
%includes longer paths (which span multiple statements)
%yields improved accuracy and successfully generalizes to different languages and tasks.

%Another work has used an NLP technique of part-of-speech (POS) tagging for programming languages purposes \cite{Binkley:2011:III:1985441.1985471}. This work has used a POS tagger on field names in programs, to tag names with POS tags such as ``noun'' and ``verb''. Based on these tags, rules were manually identified, for example ``Field names should never be only a verb''. Then, the rules could be checked on new input programs, and violations could be detected, suggesting that the field name is inadequate. This approach was only shown to detect naming violations, but not to suggest new, better names. In contrast to our approach, the detection rules in this work were manually identified, and therefore the method could not be applied to other programming languages without identifying new rules.


\para{Parse Tree Paths} An approach which resembles ours is Parse Tree Paths (PTPs) in Natural Language Processing. PTPs were mainly used in Semantic Role Labeling (SRL) --- the NLP task of identifying semantic roles such as Message, Speaker or Topic in a natural language sentence. PTPs were first suggested by \citet{gildeajurafsky2002} for automatic labeling of semantic roles, among other linguistic features. The paths were extracted from a target word to each of the constituents in question, and the method remains very popular in SRL and general NLP systems.
% A recent work in NLP~\cite{foland15} used Parse Tree Paths with convolutional neural networks, and achieved state of the art results for SRL. In addition to the traditional Parse Tree Paths, this work extended the use of path features to the dependency parse trees of natural language sentences.
The rich and unambiguous structure of programming languages renders AST paths even more important as a representation of program elements than PTPs in natural language.
\ignore{Moreover, PTPs differ from AST paths in several aspects.
A parse tree is a concrete representation of the input, and retains all the artifacts of the input, such as whitespaces and brackets. An AST is an abstract representation which keeps only the information that is relevant for prediction tasks as discussed in this paper.
%We aimed to measure the improvement we gained using several components of our approach. Most of these techniques are programming language oriented and therefore not relevant when working with natural language.
Furthermore, \textit{cross references} are unique to source code --- differently from NLP, and even when names are stripped, it is unambiguous which two identifiers refer to the same entity, which allows to use path-contexts from several occurrences of the same variable.
%Prediction of each element by itself (using all other components of our approach) relatively drops our results by 14.5\%. %  52.79%
Another difference is that PTPs are extracted in the \textit{sentence level}, while AST paths do not have such limits. The modularity of programming languages allows to extend AST paths beyond a statement level, and by limiting them to within the same block or method, allows not to capture irrelevant information.
}
%The combination between prediction of each element occurrence separately and extraction in the statement level, dropped the results dramatically in 33.59\%. % 38.3%
%The last change that we made is path extraction in the token level, using \textit{n-grams}. We used static analysis in order to determine which element is a local variable and should be predicted. Then we extracted paths sized zero to n, to both of his sides. We tested different n sizes and stopped when we got the best result, while maintaining reasonable model size (n+1 did not fit to our machine). The best result was achieved when working with 4-grams and yet, the result dropped by 7.54\% in comparison to our approach. %53.32%
%All the experiments above were conducted using the Java programming language dataset. The language choice can explain the relatively small difference from the n-grams experiment (Java is really structured language) and we believe that picking other language would yield higher differences.

\para{Code completion using PCFGs} Probabilistic Context Free Grammar (PCFG) for programming languages has been used for several tasks, such as finding code idioms~\cite{allamanis2014}.
%Such idioms can be mined by estimating the distribution of tree fragments, which also depend on the fragment size, rather than the distribution of full trees.
PCFGs were generalized by \citet{phog16} by learning a relative context node on which each production rule depends, allowing conditioning of production rules beyond the parent nonterminal, thus capturing richer context for each production rule.
%In contrast to the single context node concept, our approach uses \emph{all} of the surrounding tree nodes as a context for each prediction, taking into account the different syntactical relation to each of them.
%Another work \cite{decisionTrees2016} has extended the use of production rules with a context node, and used a decision tree algorithm to dynamically compute the context node in every step.
Even though these works use paths in an AST, they differ from our work in that the path is only used to find a context node. In our work, the path itself is part of the representation, and therefore the prediction depends not only on the context node but also on the way it is related to the element in question.

An approach for learning programs from datasets with incorrect (noisy) examples was presented by \citet{raychev2016noisy}. This approach is based on sampling the dataset and synthesizing new programs, in a feedback directed loop. %Learning is performed using empirical risk minimization (ERM). The paper presents a new approach for code completion, based on PCFG with a dynamically determined context. %The paper presents also a ``dot''-completion tool based on this approach, which exceeds the accuracy of previous systems.

\citet{tbcnn2016} used a tree-based representation to learn snippets of code using a tree-convolutional neural network, for tasks of code category classification. Our representation differs from their mainly in that we decompose the AST into paths, which better capture data-flow properties, whereas their representation decomposes into sub-trees.


==> featuregen - Copy/results-nn-table.tex <==
\begin{table}[]
\centering
\footnotesize
\begin{tabular}{ll}
\toprule
\multicolumn{1}{l}{Model} & \multicolumn{1}{l}{Names Accuracy} \\ 
\midrule
linear token-stream + word2vec    & $20.6\%$                              \\
path-neighbors, no-paths + word2vec        & $23.2\%$                              \\
\textbf{AST Paths (this work) + word2vec }                       & \textbf{40.4\%}                           \\ 
\bottomrule
\end{tabular}
\caption{Accuracy comparison for the variable name prediction task that was evaluated using word2vec in JavaScript.}
\tablabel{results-nn}
\end{table} 

==> featuregen - Copy/results-table.tex <==
\begin{table*}[]
\centering
\footnotesize
%label{my-label}
\begin{tabular}{llllr}
\toprule
Task              & \multicolumn{2}{c}{Previous works} & AST Paths (this work)   & Params (length/width)   \\ 
\midrule
\textbf{Variable name prediction} &                             &        &               \\
\tab JavaScript               & $24.9\%$ (no-paths)   & $60.0\%$ (UnuglifyJS) & \textbf{\jsacc} &  $7$/$3$          \\
\tab Java                     & $23.7\%$ (rule-based) & $50.1\%$ (CRFs$+4$-grams)& \textbf{\javaacc}               &  $6$/$3$          \\
\tab Python                   & $35.2\%$ (no-paths)   &               & \textbf{\pythonacc}             &  $7$/$4$          \\
\tab C\#                      &                       &               & \textbf{56.1\%}                 &  $7$/$4$          \\  \\
\textbf{Method name prediction} &                     &               &                        &               \\
\tab JavaScript               & $44.1\%$ (no-paths)   &               & \textbf{53.1\%}                 &  $12$/$4$         \\
\tab Java                     & \multicolumn{2}{l}{$16.5\%$, F1: $33.9$ (\citet{conv16})}             & \textbf{47.3\%}, F1: \textbf{49.9}                 &  $6$/$2$          \\
\tab Python                   & $41.6\%$ (no-paths)   &               & \textbf{51.1\%}                 &  $10$/$6$         \\  \\
\textbf{Full type prediction} &                       &               &                        &               \\
\tab Java                     & $24.1\%$ (na\"ive baseline)&          & \textbf{69.1}\% & $4$/$1$  \\
\bottomrule
\end{tabular}
\caption{Accuracy comparison for variable name prediction, method name prediction, and full type prediction using CRFs. }
%Except for the comparison to \citet{conv16} which also includes F1 score over sub-tokens, the values represent exact-match, case insensitive and ignoring non-alphabetical characters.}
\tablabel{results}
\end{table*} 

==> featuregen - Copy/semsim-table.tex <==
\begin{table}[]
\centering
\footnotesize
\begin{tabular}{c}
\begin{subtable}	[t]{.7\linewidth}
\centering
\begin{tabular}{ll}
\toprule
   & Candidate  \\ 
\midrule
1. & done           \\ 
2. & ended        \\ 
3. & complete            \\ 
4. & found      \\ 
5. & finished            \\ 
6. & stop          \\ 
7. & end             \\ 
8. & success        \\ 
\bottomrule
\end{tabular}
\caption{Candidates for prediction of the variable \scode{d} from the example program of \figref{code-example}.}
\tablabel{doneCandidates}
\end{subtable}
\\
\begin{subtable}[t]{0.7\linewidth}
\begin{tabular}{l}
\toprule
Semantic Similarities                       \\ 
\midrule
%done $\sim$ end $\sim$ ended $\sim$ complete $\sim$ finished $\sim$ stop\\
req $\sim$ request $\sim$ client                                            \\
items $\sim$ values $\sim$ objects $\sim$ keys $\sim$ elements\\
array $\sim$ arr $\sim$ ary $\sim$ list\\
item $\sim$ value $\sim$ key $\sim$ target \\
element $\sim$ elem $\sim$ el \\
count $\sim$ counter $\sim$ total \\
res $\sim$ result $\sim$ ret \\
i $\sim$ j $\sim$ index \\ 
\bottomrule
\end{tabular}
\caption{Examples of semantic similarities between names found among the top-10 candidates.}
\tablabel{topk-similarities}
\end{subtable}
\end{tabular}
\caption{Semantic similarities between names.}
\end{table} 

==> featuregen - Copy/specificmacros.tex <==
%!TEX root=draft.tex

\definecolor{airforceblue}{rgb}{0.36, 0.54, 0.66}
\definecolor{awesome}{rgb}{1.0, 0.13, 0.32}
\definecolor{blue(pigment)}{rgb}{0.2, 0.2, 0.6}
\definecolor{britishracinggreen}{rgb}{0.0, 0.26, 0.15}
\definecolor{cadmiumgreen}{rgb}{0.0, 0.42, 0.24}
\definecolor{carminered}{rgb}{1.0, 0.0, 0.22}
\definecolor{electricindigo}{rgb}{0.44, 0.0, 1.0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\hypersetup{colorlinks=true,linkcolor=blue(pigment), citecolor=cadmiumgreen, urlcolor=electricindigo}


\lstset{basicstyle=\ttfamily\scriptsize,
        language=C,
        emph={},
        emphstyle={\underbar},
        numbers=left,
        numberfirstline=false,
        numberstyle=\tiny\color{mygray},
        escapeinside={(*@}{@*)}}
\lstdefinestyle{nonumbering}{
        basicstyle=\ttfamily\scriptsize,
        language=C,
        emph={},
        emphstyle={\underbar},
        numbers=none,
        numberfirstline=false,
        numberstyle=\tiny,
        escapeinside={(*@}{@*)}
}
\lstdefinestyle{small}{
        basicstyle=\tiny,
        language=C,
        emph={},
        emphstyle={\underbar},
        numbers=none,
        numberfirstline=false,
        numberstyle=\tiny,
        escapeinside={(*@}{@*)}
}
\lstdefinelanguage
   [x64]{Assembler}     % add a "x64" dialect of Assembler
   [x86masm]{Assembler} % based on the "x86masm" dialect
   % with these extra keywords:
   {morekeywords={CDQE,CQO,CMPSQ,CMPXCHG16B,JRCXZ,LODSQ,MOVSXD, %
                  POPFQ,PUSHFQ,SCASQ,STOSQ,IRETQ,RDTSCP,SWAPGS, %
                  rax,rdx,rcx,rbx,rsi,rdi,rsp,rbp, %
                  MEM, FLAGS, FLG, assert, %
                  r9,r9d,r12,r12d,r12b, r13,r13d,r14,r14d,r15,r15d}} % etc.
\lstdefinestyle{asm}{
        basicstyle=\ttfamily\scriptsize,
        language=[x64]Assembler,
        emph={},
        emphstyle={\underbar},
        numbers=none,
        numberfirstline=false,
        numberstyle=\tiny,
        escapeinside={(*@}{@*)}
}
\lstdefinestyle{asm-small}{
        basicstyle=\ttfamily\tiny,
        language=[x64]Assembler,
        emph={},
        emphstyle={\underbar},
        numbers=none,
        numberfirstline=false,
        numberstyle=\tiny,
        escapeinside={(*@}{@*)}
}
\lstdefinestyle{asm-numbered}{
        basicstyle=\ttfamily\scriptsize,
        language=[x64]Assembler,
        emph={},
        emphstyle={\underbar},
        numbers=left,
        numberfirstline=false,
        numberstyle=\tiny\color{mygray},
        escapeinside={(*@}{@*)}
}

\usepackage{xspace} % makes sure we have spaces before next word, but not before punctuation.

\newcommand{\Boogie}{\scode{Boogie}\xspace}
\newcommand{\BoogieIR}{\scode{BoogieIVL}\xspace}
\newcommand{\IDA}{\scode{IDA Pro}\xspace}
\newcommand{\BAP}{\scode{BAP}\xspace}
\newcommand{\SMACK}{\scode{SMACK}\xspace}
\newcommand{\LLVM}{\scode{LLVM}\xspace}
\newcommand{\Python}{\scode{Python}\xspace}
\newcommand{\CSharp}{\scode{C\#}\xspace}
\newcommand{\Github}{\scode{Github}\xspace}
\newcommand{\YardPlot}{\scode{yard-plot}\xspace}
\newcommand{\BinDiff}{\scode{BinDiff}\xspace}
\newcommand{\Tracy}{\scode{TRACY}\xspace}
%\newcommand{\tool}{\scode{Esh}\xspace}
\newcommand{\website}{\href{https://github.com/tech-srl/esh}{github.com/tech-srl/esh}\xspace}
\newcommand{\Coreutils}{\scode{Coreutils}\xspace}
\newcommand{\OpenSSL}{\scode{OpenSSL}\xspace}
\newcommand{\Heartbleed}{\scode{Heartbleed}\xspace}
\newcommand{\Bash}{\scode{Bash}\xspace}
\newcommand{\Shellshock}{\scode{Shellshock}\xspace}
\newcommand{\QEMU}{\scode{QEMU}\xspace}
\newcommand{\Venom}{\scode{Venom}\xspace}
\newcommand{\gcc}{\scode{gcc}\xspace}
\newcommand{\icc}{\scode{icc}\xspace}
\newcommand{\CLang}{\scode{CLang}\xspace}
\newcommand{\Moss}{\scode{Moss}\xspace}

\newcommand{\GES}{$GES$\xspace}
\newcommand{\LES}{$LES$\xspace}
\newcommand{\VCP}{$VCP$\xspace}

\newcommand{\StrandThreshold}{5\xspace}
\newcommand{\AlphaThreshold}{0.5\xspace}
\newcommand{\QueryThreshold}{50,000\xspace}


\newcommand{\doi}[1]{doi:~\href{http://dx.doi.org/#1}{\Hurl{#1}}}   % print a hyperlinked DOI

\newcommand{\pluseq}{\mathrel{+}=}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\xcmark}{\RightDiamond}%


\def\imagetop#1{\vtop{\null\hbox{#1}}}

\newcommand{\demonsmarker}{\textbf{DEMONS START HERE IF NOT EARLIER}}

\newcommand{\sectionette}[1]{\noindent \textit{#1}:}

%\newtheorem{hypothesis}{Hypothesis}[section]
\newcommand{\hypref}[1]{Hypothesis~\ref{Hy:#1}}

\newcommand{\true}{T}
\newcommand{\false}{F}

\newcommand{\pline}[1]{#1}

\newcommand{\lnum}[1]{\textbf{#1}}
\newcommand{\reflnum}[1]{\texttt{#1}}

\newcommand{\term}[1]{\emph{#1}}

\newcommand{\authortext}[1]{{$\bullet$ \textsf{#1}}}
\newcommand{\hiddentext}[1]{}

%\newenvironment{samePageBlock}{\par
%\samepage
%}{%
%\par
%\allowbreak }

\newcommand{\para}[1]{\vspace{3pt}\noindent\textbf{\textit{#1}}}
%\newcommand{\Lparagraph}[1]{\vspace{3pt}\noindent\textit{#1.}}
\newcommand{\Lparagraph}[1]{\vspace{-4pt}\paragraph{#1}}
%\newcommand{\LLparagraph}[1]{\noindent\textit{#1.}}
\newcommand{\tab}{\hspace*{2em}}

\newcommand{\CSem}[2]{\semp{#1,#2}_{\correlate}}

\newcommand{\correlate}{\bowtie}

\newcommand{\fvar}[2]{[#1\prec #2]}

\newcommand{\better}{\sqsubseteq}
\newcommand{\wbetter}{\unlhd}

\newcommand{\sep}{\ensuremath{\ \ | \ \ }}
\newcommand{\expNum}{{1500 }}
\newcommand{\fpred}[2]{(#1\prec #2)}
\newcommand{\trans}[3]{#1\stackrel{#3}{\longrightarrow}#2}
\newcommand{\strans}[3]{#1\longrightarrow#2}
\newcommand{\mmname}{{\small \textsc{RLX}}}
\newcommand{\ebset}{\hat{E}}

\newcommand{\B}[1]{\langle{#1}\rangle}
\newcommand{\eqdef}{\buildrel \mbox{\tiny\rm def} \over =}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% notation                                        %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\optimal}{\ding{52}}
\newcommand{\success}{\ding{51}}
\newcommand{\failure}{\ding{55}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Abstraction                                     %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\eq}[1]{[#1]_{\alpha}}%{eq(#1)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Terminology                                     %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\scode}[1]{{\small \texttt{#1}}}
\newcommand{\tcode}[1]{{\scriptsize \texttt{#1}}}
\newcommand{\sname}[1]{{\small \textsc{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Actions and Traces                              %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\interseq}[1]{{\small\texttt{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Semantics                                       %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\lsyn}{\lbrack\!\lbrack}
\newcommand{\rsyn}{\rbrack\!\rbrack}
\newcommand{\semp}[1]{\lsyn #1 \rsyn}
\newcommand{\asemp}[1]{\lsyn #1 \rsyn^{\sharp}}

\newcommand{\slen}[1]{|#1|}

\newcommand{\dpless}{<_{\sigma,p}}

\newcommand{\concat}{\cdot}

%% States
\newcommand{\States}{\Sigma}
\newcommand{\sStates}{\Sigma_s}
\newcommand{\pStates}{\Sigma_p}
\newcommand{\mStates}{\Sigma_M}

%% Transitions
\newcommand{\Transitions}{\mbox{{\it \Tau}}}
\newcommand{\pTrans}{\Tau_p}
\newcommand{\mTrans}{\Tau_M}


%% Sets of States
\newcommand{\Stuck}{\mbox{{\it Stuck}}}
\newcommand{\Doomed}{\mbox{{\it Doomed}}}
\newcommand{\Initial}{\mbox{{\it Init}}}


%% Program
\newcommand{\Labels}{\italMathId{Labs}}
\newcommand{\Statements}{\italMathId{Stmts}}
\newcommand{\SharedVar}{\italMathId{Shared}}
\newcommand{\LocalVar}{\italMathId{Local}}
\newcommand{\stmt}{\mbox{{\it stmt}}}
\newcommand{\Value}{\mbox{{\it Int}}}
\newcommand{\val}[2]{\semp{#1}(#2)}
\newcommand{\Reach}{\mbox{{\it Reach}}}

%% Relations
\newcommand{\patharrow}{\rightsquigarrow}

%% General
\newcommand{\valid}{\mbox{{\it valid}}}
%\newcommand{\implies}{\Rightarrow}
\newcommand{\wgamma}{\widehat{\gamma}}
\newcommand{\powerset}{\mathcal{P}}
\newcommand{\dominatedBy}{\mbox{{\it DominatedBy}}}
\newcommand{\Ideal}{\mbox{{\it Ideal}}}
%\newcommand{\Obs}{\mbox{{\it Obs}}}
\newcommand{\Op}{\mbox{{\it Op}}} %% operations
\renewcommand{\phi}{\varphi}


\newcommand{\atomic}[2]{{\footnotesize \texttt{[#1,#2]}}}

\newcommand{\atomicmath}[2]{[#1,#2]}

\newcommand{\scheduled}{\mbox{\textit{atomic}}}
\newcommand{\nodes}{\mbox{\textit{states}}}

\newcommand{\MA}{\mbox{\textit{MA}}}

\newcommand{\aeq}{\preceq_{\alpha}}

\newcommand{\Abs}{\Sigma^{\natural}_P}
\newcommand{\Traces}{\mbox{\scode{Traces}}}

%\newcommand{\C}[1]{#1^\natural} % for all concrete symbols
\newcommand{\A}[1]{#1^\sharp} % for all abstract symbols
\newcommand{\PS}[1]{{2^{#1}}}
\newcommand{\StatesConc}{\C{C}}
\newcommand{\Formulas}{Formulas}
\newcommand{\Dom}{Dom}
\newcommand{\Below}{\sqsubseteq}
\newcommand{\violated}{Av}
\newcommand{\UStates}{\Upsilon}
\newcommand{\evalf}[2]{\llbracket #2 \rrbracket_{#1}}
\newcommand{\enf}[2]{E_{\fpred{#1}{#2}}}
\newcommand{\admits}[2]{#1\smile #2}
\newcommand{\nadmits}[2]{#1\not\smile #2}

\newcommand \abssem[1]{Abs\textsubscript{[1,#1]}}
\newcommand{\semref}[1]{Sem.~\ref{Fi:#1}}

%\newcommand{\CBS}{\cbstart}
%\newcommand{\CBE}{\cbend}

\newcommand{\CBS}{}
\newcommand{\CBE}{}


%\newcommand{\SBa}{SB1}
\newcommand{\SBb}{RA}
\newcommand{\SBc}{PDA}
\newcommand{\SBd}{OA}

\newcommand{\NoPJ}{FD}
\newcommand{\PJ}{PD}

\newcommand{\PD}[1]{{#1}^\tau}

%\newcommand{\Norm}[2]{\left\lVert{#2}\right\rVert_{#1}}
\newcommand{\Norm}[2]{VCP(#1,#2)}

% Uri: Defining colors and style for JavaScript code
\lstdefinelanguage{JavaScript}{
  keywords={break, case, catch, continue, debugger, default, delete, do, else, false, finally, for, function, if, in, instanceof, new, null, return, switch, this, throw, true, try, typeof, var, void, while, with},
  morecomment=[l]{//},
  morecomment=[s]{/*}{*/},
  morestring=[b]',
  morestring=[b]",
  ndkeywords={class, export, boolean, throw, implements, import, this},
  keywordstyle=\color{blue},
  ndkeywordstyle=\color{darkgray}\bfseries,
  identifierstyle=\color{black},
  commentstyle=\color{purple}\ttfamily,
  stringstyle=\color{red}\ttfamily,
  sensitive=true
}

\lstset{
   language=JavaScript,
   extendedchars=true,
   basicstyle=\footnotesize\ttfamily,
   showstringspaces=false,
   showspaces=false,
   %numbers=left,
   numbers=none,
   numberstyle=\footnotesize,
   numbersep=9pt,
   tabsize=2,
   breaklines=true,
   showtabs=false,
   captionpos=b
}


\newcommand{\java}{\textsc{JPredict}}
\newcommand{\js}{\textsc{JSPaths}}
\newcommand{\python}{\textsc{PythonRenamer}}
\newcommand{\tool}{\textsc{Pigeon}\xspace}
\newcommand{\maxlen}{{$max\_length$}\xspace}
\newcommand{\maxwidth}{{$max\_width$}\xspace}

\newcommand{\javaacc}{58.2\%}
\newcommand{\jsacc}{67.3\%}
\newcommand{\pythonacc}{56.7\%} 

==> featuregen - Copy/statementpath-figure.tex <==
\begin{figure}
\begin{subfigure}[b]{0.2\textwidth}
\centering
\lstset{language=JavaScript, basicstyle=\footnotesize\ttfamily,emph={fence},emphstyle=\underbar,showlines=true,escapeinside={(*@}{@*)}}

\begin{lstlisting}

var item = array[i];


\end{lstlisting}
%\caption{An example of a JavaScript statement.}
\caption{}
\label{Fi:childIdExampleLine}
\end{subfigure}
\unskip \vrule
\hspace{1mm}
\begin{subfigure}[b]{0.25\textwidth}
\centering
\includegraphics[width=1.8in]{statementPath}
%\caption{The partial AST of the statement.}
\caption{}
\label{Fi:statementPath}
\end{subfigure}
\caption{A JavaScript statement and its partial AST.}%, which demonstrates that the order of child nodes is correlated to their names.} %, and can be useful in predicting the names of other elements.}
\label{childIdExample}
\end{figure}


==> overview-figure.tex <==
\begin{figure*}
\centering
\begin{minipage}{7in}
\hspace{0.6in}
\begin{tabular}{ccc}
\begin{subfigure}[b]{0.5\textwidth}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (a){
\lstset{language=JavaScript, basicstyle=\footnotesize\ttfamily,emphstyle=\underbar,escapeinside={(*}{*)}}

\begin{lstlisting}
while (!(*\bfseries d*)) {
	if (someCondition()) {
		(*\bfseries d*) = true;
	}
}
\end{lstlisting}};
\caption{}
\figlabel{minifiedWhileOverview}
\end{subfigure}

&	
&
\hspace*{-2cm}
\begin{subfigure}[b]{0.5\textwidth}
\addtocounter{subfigure}{3}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (e){
\lstset{language=JavaScript, basicstyle=\footnotesize\ttfamily,emphstyle=\underbar,escapeinside={(*}{*)}}

\begin{lstlisting}
while (!(*\bfseries done*)) {
	if (someCondition()) {
		(*\bfseries done*) = true;
	}
}
\end{lstlisting}};
\caption{}
\label{Fi:renamedWhile}
\end{subfigure}
\\
\\
\begin{subfigure}[a]{0.5\textwidth}
\addtocounter{subfigure}{-4}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (b){\includegraphics[width=.7\linewidth, clip=true]{whileMinifiedPath}};
%\includegraphics[]{whileMinifiedPath}
\caption{}
\label{Fi:treeWhile}
\end{subfigure}
&
&
\hspace*{-2cm}
\begin{subfigure}[a]{0.5\textwidth}
\addtocounter{subfigure}{1}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (d){\includegraphics[width=.7\linewidth,clip=true]{whileCRF-word2vec}};
%\includegraphics[]{whileCRF}
\caption{}
\label{Fi:crfWhile}
\end{subfigure}
\\
\\
\\
\\
\multicolumn{3}{c}{
\begin{subfigure}[]{1\textwidth}
\scriptsize
\addtocounter{subfigure}{-2}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (c){
\begin{tabular}{@{}llll@{}}
\toprule
Identifier & Path                                                                                                                                                                       & Identifier \\ \midrule
\textbf{d}        & \textbf{SymbolRef$\uparrow$UnaryPrefix!$\uparrow$While$\downarrow$If$\downarrow$Call$\downarrow$SymbolRef}                                                                                                                                             & \textbf{someCondition}\\ \midrule
\textbf{d}        & \textbf{SymbolRef$\uparrow$UnaryPrefix!$\uparrow$While$\downarrow$If$\downarrow$Statement$\downarrow$Assign=$\downarrow$SymbolRef}~~~~~~~~~~~~~~~~~~~~~                                                                                                                                   & \textbf{d}\\ \midrule
\textbf{d}        & \textbf{SymbolRef$\uparrow$UnaryPrefix!$\uparrow$While$\downarrow$If$\downarrow$Statement$\downarrow$Assign=$\downarrow$True}                                                                                                                                             & \textbf{true}\\ \midrule
\textbf{someCondition}        & \textbf{SymbolRef$\uparrow$Call$\uparrow$If$\downarrow$Statement$\downarrow$Assign=$\downarrow$SymbolRef}                                                                                                                                             & \textbf{d}\\ \midrule
\textbf{d}        & \textbf{SymbolRef$\uparrow$Assign=$\downarrow$True}                                                                                                                                             & \textbf{true}\\ \midrule
\end{tabular}
};
%\includegraphics[]{whileMinifiedPath}
\caption{}
\tablabel{tableWhile}
\end{subfigure}
}

\end{tabular}

\tikz[remember picture,overlay]\draw[line width=2mm,-latex,gray] ([xshift=-10mm, yshift=6mm]a.south -| b.north) --node[right = 2mm,black] {\small Parse program} ([xshift=-10mm]b.north);
\tikz[remember picture,overlay]\draw[line width=2mm,-latex,gray] ([xshift=-36mm]b.south -| c.north) -- node[right = 2mm,black] {\small Extract paths} ([xshift=-36mm, yshift = 2mm]c.north);
\tikz[remember picture,overlay]\draw[line width=2mm,-latex,gray] ([xshift=-10mm, yshift = 2mm]c.north -| d.south) -- node[right = 2mm,black] {\small Learning algorithm} ([xshift=-10mm]d.south);
\tikz[remember picture,overlay]\draw[line width=2mm,-latex,gray] (d.north -| e.south) -- node[right = 2mm,black] {\small Predict} ([yshift=5mm]e.south);
\caption{An overview of the use of AST paths in learning models. A simple program (a) is parsed to construct the AST (b), from which AST paths (c) are extracted. Different learning algorithms (CRF, word2vec) can be used (d) to predict program properties. In the resulting program (e), the predicted name for \scode{d} is \scode{done}.}
\end{minipage}
\end{figure*} 
